HOMURA: Taming the Sand-Glass for Time-Constrained LLM Translation via Reinforcement Learning

Large Language Models (LLMs) have achieved remarkable strides in multilingual translation but are hindered by a systemic cross-lingual verbosity bias, rendering them unsuitable for strict time-constrained tasks like subtitling and dubbing. Current prompt-engineering approaches struggle to resolve this conflict between semantic fidelity and rigid temporal feasibility. To bridge this gap, we first introduce Sand-Glass, a benchmark specifically designed to evaluate translation under syllable-level duration constraints. Furthermore, we propose Homura, a reinforcement learning framework that explicitly optimizes the trade-off between semantic preservation and temporal compliance. By employing a constrained reinforcement learning objective featuring a novel dynamic syllable-ratio reward, Homura effectively "tames" the output length. Experimental results demonstrate that Homura significantly outperforms strong baselines, achieving precise length control that respects linguistic density hierarchies without compromising semantic adequacy.

==> section/Experiment_old.tex <==
\section{Experiments and Results}
\label{sec_experiment}

\begin{table*}[t]
    \centering
    \caption{Performance Comparison on Sand-Glass Across All Language Pairs ($\text{BLEU-$\rho$}$, $\text{Cometkiwi}$, $\text{BT-CERR}$).  All results are averaged by 3 times.}
    \label{tab:main_results_cross_lingual}
    
    \Large
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.1}

    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|ccccc|ccccc|ccccc}
        \toprule
        \multirow{3}{*}{\textbf{Model}} & \multicolumn{15}{c}{\textbf{Evaluation Metrics on Sand-Glass}} \\
        \cmidrule(lr){2-16}
         & \multicolumn{5}{c|}{\textbf{Zh $\rightarrow$ En}} & \multicolumn{5}{c|}{\textbf{Zh $\rightarrow$ De}} & \multicolumn{5}{c}{\textbf{Zh $\rightarrow$ Es}} \\
        \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
          &  \textbf{IB}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens} \\
        \midrule
        \multicolumn{16}{l}{\textit{Category 1: w/o Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  0.741  &  0.943 &  0.313 &  17.1 &  $\times$  &  0.676&  0.882 &  0.247 &  24.2 &  $\times$  &  0.668&  0.900 &  0.220 &  21.3 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.748  &  0.941 &  0.287 &  46.3 &  $\times$  &  0.676&  0.889 &  0.222 &  62.3 &  $\times$  &  0.671&  0.884 &  0.191 &  99.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  0.739  &  0.941 &  0.307 &  12.1 (916.9) &  $\times$  &  0.666&  0.877 &  0.238 &  14.2 (125.8) &  $\times$  &  0.668&  0.883 &  0.212 &  14.0 (1532.7) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  0.746  &  0.947 &  0.300 &  22.4 (412.8) &  $\times$  &  0.681&  0.894 &  0.220 &  23.2 (605.6) &  $\times$  &  0.671&  0.899 &  0.206 &  24.0 (676.8) \\

        \midrule
        \multicolumn{16}{l}{\textit{Category 2: w/ Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.691&  0.907 &  0.376&  12.2 &  $\checkmark$  &  0.535 &  0.838 &  0.293 &  17.2 &  $\times$  &  0.631&  0.849 &  0.261 &  13.5 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.700&  0.924 &  0.307 &  12.4 &  $\times$  &  0.557 &  0.866 &  0.245 &  15.8 &  $\times$  &  0.556 &  0.868 &  0.225 &  16.3 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  0.698&  0.927 &  0.322 &  10.7 (1231.3) &  $\times$  &  0.517 &  0.853 &  0.266 &  12.3 (1450.1) &  $\times$  &  0.586&  0.827 &  0.252 &  10.7 (554.5) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  0.705&  0.928 &  0.345 &  21.7 (2024.9) &  $\times$  &  0.534 &  0.874 &  0.283 &  23.1 (1962.3) &  $\times$  &  0.586&  0.833 &  0.270 &  21.0 (3105.8) \\

        \midrule
        \multicolumn{16}{l}{\textit{Category 3: Best of N}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.691&  0.903 &  0.367 &  109.7 &  $\checkmark$  &  0.611 &  0.848 &  0.324 &  109.2 &  $\checkmark$  &  0.621&  0.857 &  0.304 &  110.0 \\
        \texttt{deepseek-v3}  &  $\checkmark$  &  0.691&  0.902 &  0.332 &  122.6 &  $\checkmark$  &  0.527 &  0.863 &  0.286 &  160.5 &  $\checkmark$  &  0.522&   0.851 &  0.275 &  113.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.673&  0.904 &  0.276 &  133.2 (1089.2) &  $\checkmark$  &  0.517 &  0.854 &  0.241 &  136.0 (972.7) &  $\checkmark$  &  0.554&  0.858 &  0.235 &  133.8 (611.1) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.673&  0.906 &  0.296 &  114.2 (1810.2) &  $\checkmark$  &  0.571 &  0.861 &  0.275 &  111.2 (2229.6) &  $\checkmark$  &  0.529&  0.855 &  0.256 &  110.8 (2158.8) \\

        \midrule
        \multicolumn{16}{l}{\textit{Category 4: Translate + Modify Pipeline (2 run)}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  0.694&  0.904 &  0.327 &  30.2 &  $\times$  &  0.653&  0.868 &  0.276 &  42.7 &  $\times$  &  0.643&  0.876 &  0.246 &  37.6 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.703&  0.934 &  0.322 &  88.1 &  $\times$  &  0.645&  0.874 &  0.239 &  89.4 &  $\times$  &  0.543& 0.873 &  0.221 &  102.1 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.691&  0.902 &  0.348 &  22.3 (2517.7) &  $\times$  &  0.627&  0.830 &  0.267 &  27.5 (1043.1) &  $\checkmark$  &  0.602&  0.840 &  0.250 &  22.4 (2975.2) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.690&  0.917 &  0.321 &  42.2 (2666.2) &  $\checkmark$  &  0.514&  0.842 &  0.275 &  46.6 (2773.0) &  $\checkmark$  &  0.557&  0.820 &  0.234 &  44.9 (4012.9) \\
        \midrule
        \multicolumn{16}{l}{\textit{Category 5: HOMURA}} \\
        \midrule
        \textbf{Ours (HOMURA\textsubscript{Rubric})}  &  $\checkmark$  &  0.700 &  0.914 &  0.378 &  9.2  & $\checkmark$  & 0.591 &   0.853 &  0.317 &  16.3&   $\checkmark$ &   0.620& 0.863 &  0.260 &  13.1\\
        \textbf{Ours (HOMURA\textsubscript{Reason})}  &  $\checkmark$  &  0.701 &  0.925 &  0.376 & 10.1& $\checkmark$  & 0.603 &   0.861 &  0.321  & 14.7&  $\checkmark$ &  0.605 &  0.858 &  0.309 &  13.2 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{2mm}
    
    \raggedright
    \footnotesize
    Note: IB: In Bounds, $\checkmark$ indicates within bounds, $\times$ indicates out of bounds. AVG-Tokens: Average number of output tokens per sample; for reasoning models ($^*$), values in parentheses denote the total tokens consumed (including internal thinking).

    \vspace{-4mm}
\end{table*}

\subsection{Experimental Setup}

% \subsubsection{Translation Strategies and Baselines}
We evaluate SOTA LLMs under five strategy categories that span the length-control spectrum:

\begin{itemize}[nosep]
    \item \textbf{Category 1: Unconstrained LLMs}. Frontier models (\texttt{GPT-5}~\cite{openai2025gpt5systemcard}, \texttt{Claude-4.1-Opus}~\cite{anthropic2025claude}, \texttt{Gemini-2.5-Pro}, \texttt{DeepSeek-V3}) with standard decoding. For \texttt{GPT-5} and \texttt{Gemini-2.5-Pro}, we set low reasoning effort to approximate direct translation. These serve as semantic upper bounds.
    \item \textbf{Category 2: Prompt-based Compression.} Category 1 models with brevity-oriented system prompts enforcing syllable-level conciseness.
    \item \textbf{Category 3: Best of N Refinement.} Generating $N$ candidates with varying lengths, followed by a greedy selection of the highest-fidelity output that fulfills the syllable budget.
    \item \textbf{Category 4: Pipeline-based Post-editing.} Two-stage translation $\rightarrow$ length-constrained rewriting.
    \item \textbf{Category 5: Our Method (HOMURA).} RL fine-tuning on \texttt{Qwen3-8B}~\citep{yang2025qwen3} to enforce temporal budgets as hard constraints.
\end{itemize}

More experimental details are provided in Appendix~\ref{sec:appendix_hyper}.

\subsection{Target Syllable Bounds Configuration}
\label{ssec:target_bounds}
Following Section~\ref{sec:verbosity_bias}, we set density-calibrated target bounds $\mathcal{B}_{L}$ to impose comparable compression pressure across languages: En $\in [0.8, 0.9]$, De $\in [0.9, 1.0]$, and Es $\in [1.0, 1.1]$. These intervals are used as hard constraints for HOMURA.

\subsubsection{Evaluation Metrics}
\label{sec:evaluation_metrics}
We report complementary metrics for efficiency, semantic preservation, and linguistic quality:

\paragraph{Translation Density (BLEU-$\rho$ $\uparrow$)}
We define \textbf{BLEU-$\rho$} as semantic fidelity per temporal unit:
\begin{equation}
    \text{BLEU-}\rho = \frac{\text{BLEU}(x, \hat{x})}{\rho(x,y)},
\end{equation}
where $\text{BLEU}(x,\hat{x})$ is the back-translation BLEU~\cite{papineni2002bleu}. Since BLEU alone may not fully capture fluency in back-translation paradigms~\cite{edunov-etal-2020-evaluation}, we use BLEU-$\rho$ specifically to measure \textbf{information density}, while linguistic quality assessed via Cometkiwi.

\paragraph{Semantic Integrity (BT-CERR $\uparrow$)}
BT-CERR is a binary indicator that evaluates whether all core events extracted from $x$ are retained in the back-translation $\hat{x}$.
 (see Appendix~\ref{sec:appendix_sand-glass_construction} for the definition of core events).
% BT-CERR verifies whether core predicates and essential arguments extracted from $x$ are retained in the back-translation $\hat{x}$.

\paragraph{Linguistic Quality (Cometkiwi $\uparrow$)}
We use reference-free Cometkiwi\cite{rei2022cometkiwi} to assess fluency and adequacy under compression.

\subsection{Main Results}
\label{sec:main_results}

\subsubsection{Cross-Lingual Performance and Temporal Compliance}
\label{sec:overall_performance}

Table~\ref{tab:main_results_cross_lingual} summarizes performance on Sand-Glass. We report human evaluation in Appendix~\ref{sec:appendix_human_judgment} and Statistical Significance Testing in Appendix~\ref{sec_statistical_test_appendix}. Overall, the results highlight the trade-off between temporal compliance and semantic density:

\paragraph{Budget Violation in Frontier Models.} 
As shown by the  IB column, unconstrained frontier model(\textsc{Cat 1}) universally fail to meet temporal budgets ($\times$), particularly in low-density languages like Spanish. While specialized prompting (\textsc{Cat 2}) shifts the distribution toward brevity, it remains unreliable, with models like \texttt{GPT-5} still exhibiting "verbosity drift" that exceeds target bounds. This confirms that pure instruction-following is insufficient for rigorous syllable-level constraints.

\paragraph{The Search-Fidelity Trade-off.} 
Search-based (\textsc{Cat 3}) and pipeline (\textsc{Cat 4}) strategies achieve higher In-Bounds rates but at a significant semantic cost. For instance, \textsc{Cat 4} variants often show a drop in BT-CERR, suggesting that the disjointed post-editing process leads to "hallucinated omissions" of critical source predicates. Moreover, the increased inference latency of Best-of-$N$ makes it less practical in real-time setting.

\begin{figure*}[th]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/bt_bleu_en_comparison.pdf}
        \caption{BLEU vs. Avg. Syllable Ratio}
        \label{fig:bt_bleu}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/cerr_en_comparison.pdf}
        \caption{BT-CERR vs. Avg. Syllable Ratio}
        \label{fig:cerr_en}
    \end{subfigure}
    \caption{Quality--compression trade-off on \text{Zh}$\rightarrow$\text{En}. We plot BLEU (left) and BT-CERR (right) versus the average syllable ratio $\rho$. Each point is a model setting (marker: backbone; color: variant: Unconstrained, Rubric, GenRM, Multi-length Prompting). The red curve shows the empirical trend: quality degrades as compression strengthens.}
    
    \label{fig:tradeoff_curve}

    \vspace{-4mm}
\end{figure*}

\paragraph{Information Density Superiority of  HOMURA.} 
In contrast, HOMURA consistently maintains in bound while achieving the highest BLEU-$\rho$ across all language pairs. This gap demonstrates that HOMURA does not merely truncate text but actively performs \textit{semantic packing}—delivering a higher "semantic payload" per syllable. Additionally, we scale our method to a 32B model; see Appendix~\ref{sec:appendix_scale} for details.

\paragraph{Inference efficiency.}
HOMURA is markedly more inference-efficient. Unlike Best-of-$N$, which multiplies decoding cost by generating $N$ candidates, and unlike translate-then-modify pipelines that require an extra rewriting pass, HOMURA satisfies the syllable/temporal budget in a single decoding. Consequently, it attains high \textsc{IB} compliance with substantially fewer tokens (AVG-Tokens in Table~\ref{tab:main_results_cross_lingual}), making it suitable for real-time and high-throughput deployment.

\paragraph{Robustness of Reason-based GenRM.} 
Within Category~5, HOMURA\textsubscript{Reason} achieves higher BT-CERR than HOMURA\textsubscript{Rubric} on two of the three target languages, with the largest gain observed for English.
% Within Category~5, HOMURA\textsubscript{Reason} consistently achieves higher BT-CERR than HOMURA\textsubscript{Rubric}, with the largest gains on morphosyntactically complex targets (e.g., German). 
This suggests the reason-based reward better prunes redundancy while preserving the source’s logical structure. We further validate this by replacing the self-trained GenRM in HOMURA\textsubscript{Reason} with an LLM-as-RM baseline (\texttt{DeepSeek-V3}); results are in Appendix~\ref{sec_genrm_compare_appendix}.

\paragraph{Sensitivity of KL Regularization.}
While the theoretical objective in Eq.~\eqref{eq:kl-regularized-rl} assumes $\beta > 0$ for policy stability, our empirical investigations reveal a task-specific trade-off. 
As shown in our ablation experiments, introducing $\beta > 0$ leads to a notable degradation in structural alignment. 
This suggests that for time-constrained translation, the reference model $P_0$ imposes a ``verbosity prior'' that penalizes the radical lexical pruning and syntactic restructuring necessary to meet the Sand-Glass budget. 
By setting $\beta \to 0$ in our final implementation, we grant the model maximum \textit{compression freedom}. 
The inherent stability of the GRPO algorithm's group-relative optimization, coupled with the explicit guidance of our task-specific rewards, ensures that this relaxation preserves policy stability and prevents linguistic collapse, allowing HOMURA to reach a more efficient rate-distortion frontier. A detailed theoretical and empirical analysis of this stabilization mechanism is provided in Appendix \ref{app:stability_analysis}.

\subsubsection{Analysis of Quality--Compression Trade-off}
\label{sec:compression_tradeoff}

Figure~\ref{fig:tradeoff_curve} illustrates the trade-off between translation quality and output length. By plotting semantic metrics against the average syllable ratio $\rho$, we compare how different models perform as the available length budget decreases.

As shown in Figure~\ref{fig:tradeoff_curve}, unconstrained baselines cluster in the high-quality, high-$\rho$ region, representing the model's performance when length is not a factor. While standard LLMs can be prompted to shorten their outputs, their quality drops sharply as compression becomes more aggressive. This reflects a low rate--distortion efficiency: when forced to reduce the phonetic ``rate'' (syllables), these models suffer from disproportionately high ``distortion'' (loss of meaning), as they struggle to identify which information is most essential to preserve.

In contrast, HOMURA variants demonstrate significantly higher rate--distortion efficiency. At any given syllable budget, HOMURA maintains higher semantic fidelity than the baselines; conversely, it can achieve a much shorter length while maintaining the same quality level. These results suggest that our framework does not simply truncate text. Instead, it optimizes the model to operate at a more efficient trade-off point—packing a higher semantic payload into a limited phonetic budget to respect the strict constraints of media localization.
   
\iffalse
\subsubsection{Effect of GenRM Choice}
%\label{sec:ablation_studies}
%Table \ref{tab:ablation_study} compares HOMURA\textsubscript{Reason} with a variant that substitutes the self-trained GenRM with an external reward model implemented using DeepSeek-V3, a state-of-the-art general-purpose LLM. We report the average performance across all language pairs on three evaluation metrics.

As shown in the Table \ref{tab:ablation_study}, the compression translation model optimized with the self-trained GenRM consistently achieves better results than its counterpart using the external reward model. This indicates that a reward model trained to align with the specific objectives of compression-oriented translation provides more effective guidance during optimization. Consistent with this observation, on a held-out human-annotated reward model evaluation set designed to assess compression-aware translation quality, GenRM also demonstrates higher accuracy than the external RM, achieving 0.85 compared to 0.81. Details of the reward model evaluation set are provided in Appendix \ref{sec_genrm_test_appendix}.

\begin{table}[ht]
    \centering
    \caption{Effect of GenRM choice on compressed translation under HOMURA\textsubscript{Reason} (Average across all language pairs).}
    \label{tab:ablation_study}

    \footnotesize
    \setlength{\tabcolsep}{2.2pt}
    \renewcommand{\arraystretch}{0.95}

    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model Variant} & \textbf{BLEU-$\rho$} & \textbf{Cometkiwi} & \textbf{BT-CERR} \\
        \midrule
        HOMURA\textsubscript{Reason}  & 0.335 & 0.636 & 0.883 \\
        \midrule
        HOMURA\textsubscript{Reason} (w/ External RM)  & 0.330 &  0.628& 0.879 \\
        \bottomrule
    \end{tabular}%
    }
\end{table}
\fi

\subsubsection{Qualitative Case Studies}
\label{sec:case_studies}

We qualitatively compare HOMURA with representative baselines to assess practical behavior under different compression budgets.
As shown in Table~\ref{tab:combined_case_study}, frontier models (e.g., \texttt{GPT-5}, \texttt{Claude-4.1-opus}) often remain verbose even with brevity prompts, whereas HOMURA achieves tighter budget adherence by packing semantics into denser lexical and syntactic forms.
When the budget becomes extreme (down to $\rho \approx 0.25$), HOMURA smoothly shifts from natural prose to highly condensed translations, prioritizing core predicate--argument content while discarding redundant function words.
Full case comparisons and a taxonomy of the observed linguistic shifts are deferred to Appendix~\ref{sec:appendix_cases}.


% \subsubsection{Qualitative Case Studies}
% \label{sec:case_studies}

% To evaluate the practical efficacy of our framework, we conduct a qualitative analysis comparing HOMURA against representative baselines and examining its behavior across varying compression intensities.

% Table~\ref{tab:combined_case_study} in Appendix~\ref{sec:appendix_cases} presents a challenging \text{Zh}$\rightarrow$\text{En} instance that exemplifies the systemic \textit{verbosity bias} of frontier models. We observe that while models like \texttt{GPT-5} and \texttt{Claude-4.1} prioritize stylistic richness even with explicit prompting, HOMURA achieves precise adherence through active semantic packing. By mapping verbose syntactic structures to denser lexical equivalents (e.g., condensing a 7-syllable phrase into a 1-syllable noun), HOMURA demonstrates a superior ability to prioritize core information under strict temporal limits.

% Furthermore, our analysis of the model's tunability shows a graceful transition from natural prose to highly condensed strategies as the budget $\rho$ approaches the empirical compression limit ($\rho \approx 0.25$). In this extreme regime, HOMURA strategically prioritizes predicate-argument structures over functional redundancy, effectively navigating the trade-off between linguistic richness and feasibility. A detailed taxonomic breakdown of these linguistic shifts and the full case comparison are provided in Appendix~\ref{sec:appendix_cases}.



\subsection{Autonomous Compression: Navigating the Compression Limit}
\label{sec:auto_compression}

The preceding experiments show that HOMURA can reliably translate under a user-specified ratio interval. We further ask whether, without a preset lower bound, the model can \emph{autonomously} discover the practical compression limit: the point where additional shortening triggers a sharp loss in meaning. To this end, we formulate an autonomous compression task by replacing the hard-interval length reward with a continuous incentive:
\begin{align}
R_{\mathrm{len}}^{\mathrm{(auto)}}(x, y) = \min\left(\cos\left(\theta \cdot \rho(x, y)\right),\; 0\right),
\end{align}
where $\theta$ scales the incentive gradient. The policy is encouraged to minimize $\rho$ while still being constrained by the quality reward $R_{\mathrm{qual}}$.

\begin{table}[t] 
\centering 
\caption{The Compression Wall. The autonomous model reliably reaches the feasible limit; stricter manual targets miss $\rho$ and produce worse compression.}
\label{tab:auto_compression_results} 
\scriptsize 
\setlength{\tabcolsep}{10pt}
\begin{tabular}{lccc} \toprule 
\textbf{Model \& Configuration} & $\boldsymbol{\rho}$ & \textbf{BLEU-$\boldsymbol{\rho}$} & \textbf{BT-CERR}\\ 
\midrule \textbf{Auto HOMURA} & \textbf{0.485} & 0.404 & 0.811 \\ 
% \textbf{Auto HOMURA\textsubscript{Reason}} & \textbf{0.459} & 0.390 & 0.805\\ 
\midrule \multicolumn{4}{l}{\textit{Manually Constrained HOMURA}} \\ 
\hspace{1mm} $R_{\mathrm{target}} \in [0.3, 0.4]$ & 0.558 & 0.392 & 0.819\\
\hspace{1mm} $R_{\mathrm{target}} \in [0.4, 0.5]$ & \textbf{0.481} & 0.384 & 0.816\\ 
\hspace{1mm} $R_{\mathrm{target}} \in [0.5, 0.6]$ & 0.559 & 0.386 & 0.856\\
\hspace{1mm} $R_{\mathrm{target}} \in [0.8, 0.9]$ & 0.808 & 0.378 & 0.914\\ 
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

% \paragraph{The Empirical Compression Wall}

% A consistent \textit{compression wall} emerges when the model is pushed toward its structural limits. As shown in Table~\ref{tab:auto_compression_results}, when optimized autonomously, the model converges to a stable average ratio of $\rho \approx 0.485$. 

% Notably, even when we impose an \textit{ultra-aggressive target bound} of $[0.3, 0.4]$---a range that likely exceeds the theoretical limit of information density---the model fails to reach shorter lengths. Instead, the achieved ratio regresses to $\rho=0.558$, accompanied by a severe drop in semantic coherence. This non-linear response suggests that $\rho \approx 0.49$ represents a \textit{critical feasibility threshold} for Zh-to-En translation. Any attempt to compress beyond this ``wall'' triggers a conflict between length and quality rewards, where the model can no longer maintain basic syntax while staying brief.

\paragraph{The Empirical Compression Wall}

We observe a stable \textit{compression wall} when pushing the model to its structural limit. In Table~\ref{tab:auto_compression_results}, autonomous optimization consistently converges to a narrow operating regime around $\rho \in [0.46, 0.49]$, regardless of the specific reward configuration.

When we enforce an ultra-aggressive target of $[0.3, 0.4]$, the model does \emph{not} become shorter; instead it rebounds to $\rho=0.558$ and semantic coherence collapses. This non-linear failure indicates a feasibility threshold around $\rho \approx 0.49$ for Zh$\rightarrow$En: compressing beyond it creates an irreconcilable length-quality trade-off, where the model cannot preserve basic well-formedness while remaining brief.

\paragraph{Efficiency at the Frontier}
To quantify compression efficiency, we report BLEU-$\rho$. The autonomous model attains the best BLEU-$\rho$ while operating at a genuinely shorter length ($\rho=0.485$ vs.\ $0.558$), indicating that autonomous optimization finds a more efficient operating point on the quality-compression frontier.

\paragraph{Rate-Distortion Efficiency at the Frontier}
Qualitatively, the autonomous model tends to compress by \emph{semantic condensation}: dropping modifiers, selecting denser lexical items, and simplifying clause structures. In contrast, when forced toward an overly aggressive interval, outputs more often exhibit unstable shortening behaviors, reflecting the tension between further length reduction and preserving core meaning.

\paragraph{Takeaway: The Wall as a Feasibility Boundary}
Together, these results suggest an empirical feasibility boundary around $\rho\approx0.49$ for time-constrained translation in our setting (Zh→En).% This empirical limit closely aligns with the theoretical density floor predicted by the Iso-Information Principle introduced in Section \ref{sec:verbosity_bias}.
We hypothesize that this boundary represents the minimal information carrier required to express core predicate-argument content.


==> section_backup_old/Conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

We address systemic cross-lingual verbosity bias in LLM translation, a key obstacle in time-constrained settings such as subtitles and dubbing. We introduce Sand-Glass, a syllable-budgeted benchmark grounded in the Iso-Information Principle, and propose HOMURA, an RL framework that optimizes the fidelity--feasibility trade-off.

With a KL-regularized objective and a dynamic syllable-ratio reward, HOMURA achieves strict length compliance without reference translations while improving information density (BLEU-$\rho$). Future work will test whether the observed compression feasibility boundary (e.g., $\rho \approx 0.49$ for Zh$\rightarrow$En) generalizes across language pairs, and extend HOMURA to end-to-end speech translation with joint semantic and duration optimization.

% \section{Conclusion} 
% \label{sec:conclusion} 
% In this paper, we tackle systemic cross-lingual verbosity bias in LLM translation, which limits deployment in time-constrained settings (e.g., subtitles and dubbing). We introduce Sand-Glass, a benchmark with syllable-level duration budgets grounded in the Iso-Information Principle, and propose HOMURA, an RL framework that directly optimizes the fidelity--feasibility trade-off. 

% Using a KL-regularized objective and a dynamic syllable-ratio reward, HOMURA learns to satisfy strict length constraints without reference translations. Experiments show that it markedly improves compliance while increasing information density (BLEU-$\rho$), enabling efficient semantic packing rather than naive truncation. Future work will investigate the universality of the empirical `compression feasibility boundary'' (observed around $\rho \approx 0.49$ for Zh->En) across diverse language pairs. 

% Furthermore, we aim to extend this framework to end-to-end speech translation, exploring how to jointly optimize semantic fidelity and prosodic duration for precise synchronization in real-time scenarios.

==> section_backup_old/Experiment.tex <==
\section{Experiments and Results}
\label{sec_experiment}

\begin{table*}[t]
    \centering
    \caption{Performance Comparison on Sand-Glass Across All Language Pairs ($\text{BLEU-$\rho$}$, $\text{Cometkiwi}$, $\text{BT-CERR}$).  All results are averaged by 3 times.}
    \label{tab:main_results_cross_lingual}
    
    \Large
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.1}

    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|cccccc|cccccc|cccccc}
        \toprule
        \multirow{3}{*}{\textbf{Model}} & \multicolumn{18}{c}{\textbf{Evaluation Metrics on Sand-Glass}} \\
        \cmidrule(lr){2-19}
         & \multicolumn{6}{c|}{\textbf{Zh $\rightarrow$ En}} & \multicolumn{6}{c|}{\textbf{Zh $\rightarrow$ De}} & \multicolumn{6}{c}{\textbf{Zh $\rightarrow$ Es}} \\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
          &  \textbf{IB}  &  \textbf{syllable-ratio}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{syllable-ratio}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{syllable-ratio}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens} \\
        \midrule
        \multicolumn{19}{l}{\textit{Category 1: w/o Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  1.361  &  0.741  &  0.943 &  0.313 &  17.1 &  $\times$  &  1.582  &  0.676&  0.882 &  0.247 &  24.2 &  $\times$  &  1.812  &  0.668&  0.900 &  0.220 &  21.3 \\
        \texttt{deepseek-v3}  &  $\times$  &  1.413  &  0.748  &  0.941 &  0.287 &  46.3 &  $\times$  &  1.669  &  0.676&  0.889 &  0.222 &  62.3 &  $\times$  &  1.993  &  0.671&  0.884 &  0.191 &  99.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  1.289  &  0.739  &  0.941 &  0.307 &  12.1 (916.9) &  $\times$  &  1.512  &  0.666&  0.877 &  0.238 &  14.2 (125.8) &  $\times$  &  1.719  &  0.668&  0.883 &  0.212 &  14.0 (1532.7) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  1.330  &  0.746  &  0.947 &  0.300 &  22.4 (412.8) &  $\times$  &  1.633  &  0.681&  0.894 &  0.220 &  23.2 (605.6) &  $\times$  &  1.864  &  0.671&  0.899 &  0.206 &  24.0 (676.8) \\

        \midrule
        \multicolumn{19}{l}{\textit{Category 2: w/ Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.852  &  0.691&  0.907 &  0.376&  12.2 &  $\checkmark$  &  0.951  &  0.535 &  0.838 &  0.293 &  17.2 &  $\times$  &  1.106  &  0.631&  0.849 &  0.261 &  13.5 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.960  &  0.700&  0.924 &  0.307 &  12.4 &  $\times$  &  1.196  &  0.557 &  0.866 &  0.245 &  15.8 &  $\times$  &  1.355  &  0.556 &  0.868 &  0.225 &  16.3 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  0.920  &  0.698&  0.927 &  0.322 &  10.7 (1231.3) &  $\times$  &  1.016  &  0.517 &  0.853 &  0.266 &  12.3 (1450.1) &  $\times$  &  0.974  &  0.586&  0.827 &  0.252 &  10.7 (554.5) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  0.937  &  0.705&  0.928 &  0.345 &  21.7 (2024.9) &  $\times$  &  1.025  &  0.534 &  0.874 &  0.283 &  23.1 (1962.3) &  $\times$  &  0.982  &  0.586&  0.833 &  0.270 &  21.0 (3105.8) \\

        \midrule
        \multicolumn{19}{l}{\textit{Category 3: Best of N}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.845  &  0.691&  0.903 &  0.367 &  109.7 &  $\checkmark$  &  0.946  &  0.611 &  0.848 &  0.324 &  109.2 &  $\checkmark$  &  1.039  &  0.621&  0.857 &  0.304 &  110.0 \\
        \texttt{deepseek-v3}  &  $\checkmark$  &  0.852  &  0.691&  0.902 &  0.332 &  122.6 &  $\checkmark$  &  0.959  &  0.527 &  0.863 &  0.286 &  160.5 &  $\checkmark$  &  1.042  &  0.522&   0.851 &  0.275 &  113.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.900  &  0.673&  0.904 &  0.276 &  133.2 (1089.2) &  $\checkmark$  &  0.992  &  0.517 &  0.854 &  0.241 &  136.0 (972.7) &  $\checkmark$  &  1.087  &  0.554&  0.858 &  0.235 &  133.8 (611.1) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.888  &  0.673&  0.906 &  0.296 &  114.2 (1810.2) &  $\checkmark$  &  0.994  &  0.571 &  0.861 &  0.275 &  111.2 (2229.6) &  $\checkmark$  &  1.076  &  0.529&  0.855 &  0.256 &  110.8 (2158.8) \\

        \midrule
        \multicolumn{19}{l}{\textit{Category 4: Translate + Modify Pipeline (2 run)}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  0.918  &  0.694&  0.904 &  0.327 &  30.2 &  $\times$  &  1.089  &  0.653&  0.868 &  0.276 &  42.7 &  $\times$  &  1.284  &  0.643&  0.876 &  0.246 &  37.6 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.967  &  0.703&  0.934 &  0.322 &  88.1 &  $\times$  &  1.154  &  0.645&  0.874 &  0.239 &  89.4 &  $\times$  &  1.301  &  0.543& 0.873 &  0.221 &  102.1 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.837  &  0.691&  0.902 &  0.348 &  22.3 (2517.7) &  $\times$  &  1.001  &  0.627&  0.830 &  0.267 &  27.5 (1043.1) &  $\checkmark$  &  1.042  &  0.602&  0.840 &  0.250 &  22.4 (2975.2) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.833  &  0.690&  0.917 &  0.321 &  42.2 (2666.2) &  $\checkmark$  &  0.934  &  0.514&  0.842 &  0.275 &  46.6 (2773.0) &  $\checkmark$  &  1.018  &  0.557&  0.820 &  0.234 &  44.9 (4012.9) \\
        \midrule
        \multicolumn{19}{l}{\textit{Category 5: HOMURA}} \\
        \midrule
        \textbf{Ours (HOMURA\textsubscript{Rubric})}  &  $\checkmark$  & 0.809 &  0.700 &  0.914 &  0.378 &  9.2  & $\checkmark$  & 0.960 & 0.591 &   0.853 &  0.317 &  16.3&   $\checkmark$ & 1.067 &   0.620& 0.863 &  0.260 &  13.1 \\
        \textbf{Ours (HOMURA\textsubscript{Reason})}  &  $\checkmark$  &  0.846 &  0.701 &  0.925 &  0.376 & 10.1& $\checkmark$  & 0.918 & 0.603 &   0.861 &  0.321  & 14.7&  $\checkmark$ & 1.057 & 0.605 &  0.858 &  0.309 &  13.2 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{2mm}
    
    \raggedright
    \footnotesize
    Note: IB: In Bounds, $\checkmark$ indicates within bounds, $\times$ indicates out of bounds. AVG-Tokens: Average number of output tokens per sample; for reasoning models ($^*$), values in parentheses denote the total tokens consumed (including internal thinking).

    \vspace{-4mm}
\end{table*}

\subsection{Experimental Setup}

% \subsubsection{Translation Strategies and Baselines}
We evaluate SOTA LLMs under five strategy categories that span the length-control spectrum:

\begin{itemize}[nosep]
    \item \textbf{Category 1: Unconstrained LLMs}. Frontier models (\texttt{GPT-5}~\cite{openai2025gpt5systemcard}, \texttt{Claude-4.1-Opus}~\cite{anthropic2025claude}, \texttt{Gemini-2.5-Pro}, \texttt{DeepSeek-V3}) with standard decoding. For \texttt{GPT-5} and \texttt{Gemini-2.5-Pro}, we set low reasoning effort to approximate direct translation. These serve as semantic upper bounds.
    \item \textbf{Category 2: Prompt-based Compression.} Category 1 models with brevity-oriented system prompts enforcing syllable-level conciseness.
    \item \textbf{Category 3: Best of N Refinement.} Generating $N$ candidates with varying lengths, followed by a greedy selection of the highest-fidelity output that fulfills the syllable budget.
    \item \textbf{Category 4: Pipeline-based Post-editing.} Two-stage translation $\rightarrow$ length-constrained rewriting.
    \item \textbf{Category 5: Our Method (HOMURA).} RL fine-tuning on \texttt{Qwen3-8B}~\citep{yang2025qwen3} to enforce temporal budgets as hard constraints.
\end{itemize}

More experimental details are provided in Appendix~\ref{sec:appendix_hyper}.

\subsection{Target Syllable Bounds Configuration}
\label{ssec:target_bounds}
Following Section~\ref{sec:verbosity_bias}, we set density-calibrated target bounds $\mathcal{B}_{L}$ to impose comparable compression pressure across languages: En $\in [0.8, 0.9]$, De $\in [0.9, 1.0]$, and Es $\in [1.0, 1.1]$. These intervals are used as hard constraints for HOMURA.

\subsubsection{Evaluation Metrics}
\label{sec:evaluation_metrics}
We report complementary metrics for efficiency, semantic preservation, and linguistic quality:

\paragraph{Translation Density (BLEU-$\rho$ $\uparrow$)}
We define \textbf{BLEU-$\rho$} as semantic fidelity per temporal unit:
\begin{equation}
    \text{BLEU-}\rho = \frac{\text{BLEU}(x, \hat{x})}{\rho(x,y)},
\end{equation}
where $\text{BLEU}(x,\hat{x})$ is the back-translation BLEU~\cite{papineni2002bleu}. Since BLEU alone may not fully capture fluency in back-translation paradigms~\cite{edunov-etal-2020-evaluation}, we use BLEU-$\rho$ specifically to measure \textbf{information density}, while linguistic quality assessed via Cometkiwi.

\paragraph{Semantic Integrity (BT-CERR $\uparrow$)}
BT-CERR is a binary indicator that evaluates whether all core events extracted from $x$ are retained in the back-translation $\hat{x}$.
 (see Appendix~\ref{sec:appendix_sand-glass_construction} for the definition of core events).
% BT-CERR verifies whether core predicates and essential arguments extracted from $x$ are retained in the back-translation $\hat{x}$.

\paragraph{Linguistic Quality (Cometkiwi $\uparrow$)}
We use reference-free Cometkiwi\cite{rei2022cometkiwi} to assess fluency and adequacy under compression.

\subsection{Main Results}
\label{sec:main_results}

\subsubsection{Cross-Lingual Performance and Temporal Compliance}
\label{sec:overall_performance}

Table~\ref{tab:main_results_cross_lingual} summarizes performance on Sand-Glass. We report human evaluation in Appendix~\ref{sec:appendix_human_judgment} and Statistical Significance Testing in Appendix~\ref{sec_statistical_test_appendix}. Overall, the results highlight the trade-off between temporal compliance and semantic density:

\paragraph{Budget Violation in Frontier Models.} 
As shown by the  IB column, unconstrained frontier model(\textsc{Cat 1}) universally fail to meet temporal budgets ($\times$), particularly in low-density languages like Spanish. While specialized prompting (\textsc{Cat 2}) shifts the distribution toward brevity, it remains unreliable, with models like \texttt{GPT-5} still exhibiting "verbosity drift" that exceeds target bounds. This confirms that pure instruction-following is insufficient for rigorous syllable-level constraints.

\paragraph{The Search-Fidelity Trade-off.} 
Search-based (\textsc{Cat 3}) and pipeline (\textsc{Cat 4}) strategies achieve higher In-Bounds rates but at a significant semantic cost. For instance, \textsc{Cat 4} variants often show a drop in BT-CERR, suggesting that the disjointed post-editing process leads to "hallucinated omissions" of critical source predicates. Moreover, the increased inference latency of Best-of-$N$ makes it less practical in real-time setting.

\begin{figure*}[th]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/bt_bleu_en_comparison.pdf}
        \caption{BLEU vs. Avg. Syllable Ratio}
        \label{fig:bt_bleu}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/cerr_en_comparison.pdf}
        \caption{BT-CERR vs. Avg. Syllable Ratio}
        \label{fig:cerr_en}
    \end{subfigure}
    \caption{Quality--compression trade-off on \text{Zh}$\rightarrow$\text{En}. We plot BLEU (left) and BT-CERR (right) versus the average syllable ratio $\rho$. Each point is a model setting (marker: backbone; color: variant: Unconstrained, Rubric, GenRM, Multi-length Prompting). The red curve shows the empirical trend: quality degrades as compression strengthens.}
    
    \label{fig:tradeoff_curve}

    \vspace{-4mm}
\end{figure*}

\paragraph{Information Density Superiority of  HOMURA.} 
In contrast, HOMURA consistently maintains in bound while achieving the highest BLEU-$\rho$ across all language pairs. This gap demonstrates that HOMURA does not merely truncate text but actively performs \textit{semantic packing}—delivering a higher "semantic payload" per syllable. Additionally, we scale our method to a 32B model; see Appendix~\ref{sec:appendix_scale} for details.

\paragraph{Inference efficiency.}
HOMURA is markedly more inference-efficient. Unlike Best-of-$N$, which multiplies decoding cost by generating $N$ candidates, and unlike translate-then-modify pipelines that require an extra rewriting pass, HOMURA satisfies the syllable/temporal budget in a single decoding. Consequently, it attains high \textsc{IB} compliance with substantially fewer tokens (AVG-Tokens in Table~\ref{tab:main_results_cross_lingual}), making it suitable for real-time and high-throughput deployment.

\paragraph{Robustness of Reason-based GenRM.} 
Within Category~5, HOMURA\textsubscript{Reason} achieves higher BT-CERR than HOMURA\textsubscript{Rubric} on two of the three target languages, with the largest gain observed for English.
% Within Category~5, HOMURA\textsubscript{Reason} consistently achieves higher BT-CERR than HOMURA\textsubscript{Rubric}, with the largest gains on morphosyntactically complex targets (e.g., German). 
This suggests the reason-based reward better prunes redundancy while preserving the source’s logical structure. We further validate this by replacing the self-trained GenRM in HOMURA\textsubscript{Reason} with an LLM-as-RM baseline (\texttt{DeepSeek-V3}); results are in Appendix~\ref{sec_genrm_compare_appendix}.

\paragraph{Sensitivity of KL Regularization.}
While the theoretical objective in Eq.~\eqref{eq:kl-regularized-rl} assumes $\beta > 0$ for policy stability, our empirical investigations reveal a task-specific trade-off. 
As shown in our ablation experiments, introducing $\beta > 0$ leads to a notable degradation in structural alignment. 
This suggests that for time-constrained translation, the reference model $P_0$ imposes a ``verbosity prior'' that penalizes the radical lexical pruning and syntactic restructuring necessary to meet the Sand-Glass budget. 
By setting $\beta \to 0$ in our final implementation, we grant the model maximum \textit{compression freedom}. 
The inherent stability of the GRPO algorithm's group-relative optimization, coupled with the explicit guidance of our task-specific rewards, ensures that this relaxation preserves policy stability and prevents linguistic collapse, allowing HOMURA to reach a more efficient rate-distortion frontier. A detailed theoretical and empirical analysis of this stabilization mechanism is provided in Appendix \ref{app:stability_analysis}.

\subsubsection{Analysis of Quality--Compression Trade-off}
\label{sec:compression_tradeoff}

Figure~\ref{fig:tradeoff_curve} illustrates the trade-off between translation quality and output length. By plotting semantic metrics against the average syllable ratio $\rho$, we compare how different models perform as the available length budget decreases.

As shown in Figure~\ref{fig:tradeoff_curve}, unconstrained baselines cluster in the high-quality, high-$\rho$ region, representing the model's performance when length is not a factor. While standard LLMs can be prompted to shorten their outputs, their quality drops sharply as compression becomes more aggressive. This reflects a low rate--distortion efficiency: when forced to reduce the phonetic ``rate'' (syllables), these models suffer from disproportionately high ``distortion'' (loss of meaning), as they struggle to identify which information is most essential to preserve.

In contrast, HOMURA variants demonstrate significantly higher rate--distortion efficiency. At any given syllable budget, HOMURA maintains higher semantic fidelity than the baselines; conversely, it can achieve a much shorter length while maintaining the same quality level. These results suggest that our framework does not simply truncate text. Instead, it optimizes the model to operate at a more efficient trade-off point—packing a higher semantic payload into a limited phonetic budget to respect the strict constraints of media localization.
   
\iffalse
\subsubsection{Effect of GenRM Choice}
%\label{sec:ablation_studies}
%Table \ref{tab:ablation_study} compares HOMURA\textsubscript{Reason} with a variant that substitutes the self-trained GenRM with an external reward model implemented using DeepSeek-V3, a state-of-the-art general-purpose LLM. We report the average performance across all language pairs on three evaluation metrics.

As shown in the Table \ref{tab:ablation_study}, the compression translation model optimized with the self-trained GenRM consistently achieves better results than its counterpart using the external reward model. This indicates that a reward model trained to align with the specific objectives of compression-oriented translation provides more effective guidance during optimization. Consistent with this observation, on a held-out human-annotated reward model evaluation set designed to assess compression-aware translation quality, GenRM also demonstrates higher accuracy than the external RM, achieving 0.85 compared to 0.81. Details of the reward model evaluation set are provided in Appendix \ref{sec_genrm_test_appendix}.

\begin{table}[ht]
    \centering
    \caption{Effect of GenRM choice on compressed translation under HOMURA\textsubscript{Reason} (Average across all language pairs).}
    \label{tab:ablation_study}

    \footnotesize
    \setlength{\tabcolsep}{2.2pt}
    \renewcommand{\arraystretch}{0.95}

    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model Variant} & \textbf{BLEU-$\rho$} & \textbf{Cometkiwi} & \textbf{BT-CERR} \\
        \midrule
        HOMURA\textsubscript{Reason}  & 0.335 & 0.636 & 0.883 \\
        \midrule
        HOMURA\textsubscript{Reason} (w/ External RM)  & 0.330 &  0.628& 0.879 \\
        \bottomrule
    \end{tabular}%
    }
\end{table}
\fi

\subsubsection{Qualitative Case Studies}
\label{sec:case_studies}

We qualitatively compare \textsc{Homura} against three baseline strategies built on a frontier LLM (Claude-4.1-Opus): unconstrained translation, hard truncation, and best-of-$N$ refinement with $k{=}4$ candidates.
As shown in Table~\ref{tab:case_study}, the unconstrained baseline consistently over-translates ($\rho > 1.2$), and hard truncation to the syllable budget produces syntactically broken sentences that end mid-phrase.
The best-of-$N$ approach generates candidates spanning a wide ratio range, yet adjacent candidates exhibit a characteristic \emph{cliff pattern}---jumping from above the target interval to well below it---leaving the $[0.8, 0.9]$ window uncovered.
\textsc{Homura}, by contrast, hits the target ratio in a single decoding pass while preserving both grammatical completeness and the pragmatic register of the source.
Full case details and analysis are provided in Appendix~\ref{sec:appendix_cases}.


% \subsubsection{Qualitative Case Studies}
% \label{sec:case_studies}

% To evaluate the practical efficacy of our framework, we conduct a qualitative analysis comparing HOMURA against representative baselines and examining its behavior across varying compression intensities.

% Table~\ref{tab:combined_case_study} in Appendix~\ref{sec:appendix_cases} presents a challenging \text{Zh}$\rightarrow$\text{En} instance that exemplifies the systemic \textit{verbosity bias} of frontier models. We observe that while models like \texttt{GPT-5} and \texttt{Claude-4.1} prioritize stylistic richness even with explicit prompting, HOMURA achieves precise adherence through active semantic packing. By mapping verbose syntactic structures to denser lexical equivalents (e.g., condensing a 7-syllable phrase into a 1-syllable noun), HOMURA demonstrates a superior ability to prioritize core information under strict temporal limits.

% Furthermore, our analysis of the model's tunability shows a graceful transition from natural prose to highly condensed strategies as the budget $\rho$ approaches the empirical compression limit ($\rho \approx 0.25$). In this extreme regime, HOMURA strategically prioritizes predicate-argument structures over functional redundancy, effectively navigating the trade-off between linguistic richness and feasibility. A detailed taxonomic breakdown of these linguistic shifts and the full case comparison are provided in Appendix~\ref{sec:appendix_cases}.



\subsection{Autonomous Compression: Navigating the Compression Limit}
\label{sec:auto_compression}

The preceding experiments show that HOMURA can reliably translate under a user-specified ratio interval. We further ask whether, without a preset lower bound, the model can \emph{autonomously} discover the practical compression limit: the point where additional shortening triggers a sharp loss in meaning. To this end, we formulate an autonomous compression task by replacing the hard-interval length reward with a continuous incentive:
\begin{align}
R_{\mathrm{len}}^{\mathrm{(auto)}}(x, y) = \min\left(\cos\left(\theta \cdot \rho(x, y)\right),\; 0\right),
\end{align}
where $\theta$ scales the incentive gradient. The policy is encouraged to minimize $\rho$ while still being constrained by the quality reward $R_{\mathrm{qual}}$.

\begin{table}[t] 
\centering 
\caption{The Compression Wall. The autonomous model reliably reaches the feasible limit; stricter manual targets miss $\rho$ and produce worse compression.}
\label{tab:auto_compression_results} 
\scriptsize 
\setlength{\tabcolsep}{10pt}
\begin{tabular}{lccc} \toprule 
\textbf{Model \& Configuration} & $\boldsymbol{\rho}$ & \textbf{BLEU-$\boldsymbol{\rho}$} & \textbf{BT-CERR}\\ 
\midrule \textbf{Auto HOMURA} & \textbf{0.485} & 0.404 & 0.811 \\ 
% \textbf{Auto HOMURA\textsubscript{Reason}} & \textbf{0.459} & 0.390 & 0.805\\ 
\midrule \multicolumn{4}{l}{\textit{Manually Constrained HOMURA}} \\ 
\hspace{1mm} $R_{\mathrm{target}} \in [0.3, 0.4]$ & 0.558 & 0.392 & 0.819\\
\hspace{1mm} $R_{\mathrm{target}} \in [0.4, 0.5]$ & \textbf{0.481} & 0.384 & 0.816\\ 
\hspace{1mm} $R_{\mathrm{target}} \in [0.5, 0.6]$ & 0.559 & 0.386 & 0.856\\
\hspace{1mm} $R_{\mathrm{target}} \in [0.8, 0.9]$ & 0.808 & 0.378 & 0.914\\ 
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

% \paragraph{The Empirical Compression Wall}

% A consistent \textit{compression wall} emerges when the model is pushed toward its structural limits. As shown in Table~\ref{tab:auto_compression_results}, when optimized autonomously, the model converges to a stable average ratio of $\rho \approx 0.485$. 

% Notably, even when we impose an \textit{ultra-aggressive target bound} of $[0.3, 0.4]$---a range that likely exceeds the theoretical limit of information density---the model fails to reach shorter lengths. Instead, the achieved ratio regresses to $\rho=0.558$, accompanied by a severe drop in semantic coherence. This non-linear response suggests that $\rho \approx 0.49$ represents a \textit{critical feasibility threshold} for Zh-to-En translation. Any attempt to compress beyond this ``wall'' triggers a conflict between length and quality rewards, where the model can no longer maintain basic syntax while staying brief.

\paragraph{The Empirical Compression Wall}

We observe a stable \textit{compression wall} when pushing the model to its structural limit. In Table~\ref{tab:auto_compression_results}, autonomous optimization consistently converges to a narrow operating regime around $\rho \in [0.46, 0.49]$, regardless of the specific reward configuration.

When we enforce an ultra-aggressive target of $[0.3, 0.4]$, the model does \emph{not} become shorter; instead it rebounds to $\rho=0.558$ and semantic coherence collapses. This non-linear failure indicates a feasibility threshold around $\rho \approx 0.49$ for Zh$\rightarrow$En: compressing beyond it creates an irreconcilable length-quality trade-off, where the model cannot preserve basic well-formedness while remaining brief.

\paragraph{Efficiency at the Frontier}
To quantify compression efficiency, we report BLEU-$\rho$. The autonomous model attains the best BLEU-$\rho$ while operating at a genuinely shorter length ($\rho=0.485$ vs.\ $0.558$), indicating that autonomous optimization finds a more efficient operating point on the quality-compression frontier.

\paragraph{Rate-Distortion Efficiency at the Frontier}
Qualitatively, the autonomous model tends to compress by \emph{semantic condensation}: dropping modifiers, selecting denser lexical items, and simplifying clause structures. In contrast, when forced toward an overly aggressive interval, outputs more often exhibit unstable shortening behaviors, reflecting the tension between further length reduction and preserving core meaning.

\paragraph{Takeaway: The Wall as a Feasibility Boundary}
Together, these results suggest an empirical feasibility boundary around $\rho\approx0.49$ for time-constrained translation in our setting (Zh→En).% This empirical limit closely aligns with the theoretical density floor predicted by the Iso-Information Principle introduced in Section \ref{sec:verbosity_bias}.
We hypothesize that this boundary represents the minimal information carrier required to express core predicate-argument content.


==> section_backup_old/Experiment_old.tex <==
\section{Experiments and Results}
\label{sec_experiment}

\begin{table*}[t]
    \centering
    \caption{Performance Comparison on Sand-Glass Across All Language Pairs ($\text{BLEU-$\rho$}$, $\text{Cometkiwi}$, $\text{BT-CERR}$).  All results are averaged by 3 times.}
    \label{tab:main_results_cross_lingual}
    
    \Large
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.1}

    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|ccccc|ccccc|ccccc}
        \toprule
        \multirow{3}{*}{\textbf{Model}} & \multicolumn{15}{c}{\textbf{Evaluation Metrics on Sand-Glass}} \\
        \cmidrule(lr){2-16}
         & \multicolumn{5}{c|}{\textbf{Zh $\rightarrow$ En}} & \multicolumn{5}{c|}{\textbf{Zh $\rightarrow$ De}} & \multicolumn{5}{c}{\textbf{Zh $\rightarrow$ Es}} \\
        \cmidrule(lr){2-6} \cmidrule(lr){7-11} \cmidrule(lr){12-16}
          &  \textbf{IB}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens} \\
        \midrule
        \multicolumn{16}{l}{\textit{Category 1: w/o Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  0.741  &  0.943 &  0.313 &  17.1 &  $\times$  &  0.676&  0.882 &  0.247 &  24.2 &  $\times$  &  0.668&  0.900 &  0.220 &  21.3 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.748  &  0.941 &  0.287 &  46.3 &  $\times$  &  0.676&  0.889 &  0.222 &  62.3 &  $\times$  &  0.671&  0.884 &  0.191 &  99.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  0.739  &  0.941 &  0.307 &  12.1 (916.9) &  $\times$  &  0.666&  0.877 &  0.238 &  14.2 (125.8) &  $\times$  &  0.668&  0.883 &  0.212 &  14.0 (1532.7) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  0.746  &  0.947 &  0.300 &  22.4 (412.8) &  $\times$  &  0.681&  0.894 &  0.220 &  23.2 (605.6) &  $\times$  &  0.671&  0.899 &  0.206 &  24.0 (676.8) \\

        \midrule
        \multicolumn{16}{l}{\textit{Category 2: w/ Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.691&  0.907 &  0.376&  12.2 &  $\checkmark$  &  0.535 &  0.838 &  0.293 &  17.2 &  $\times$  &  0.631&  0.849 &  0.261 &  13.5 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.700&  0.924 &  0.307 &  12.4 &  $\times$  &  0.557 &  0.866 &  0.245 &  15.8 &  $\times$  &  0.556 &  0.868 &  0.225 &  16.3 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  0.698&  0.927 &  0.322 &  10.7 (1231.3) &  $\times$  &  0.517 &  0.853 &  0.266 &  12.3 (1450.1) &  $\times$  &  0.586&  0.827 &  0.252 &  10.7 (554.5) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  0.705&  0.928 &  0.345 &  21.7 (2024.9) &  $\times$  &  0.534 &  0.874 &  0.283 &  23.1 (1962.3) &  $\times$  &  0.586&  0.833 &  0.270 &  21.0 (3105.8) \\

        \midrule
        \multicolumn{16}{l}{\textit{Category 3: Best of N}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.691&  0.903 &  0.367 &  109.7 &  $\checkmark$  &  0.611 &  0.848 &  0.324 &  109.2 &  $\checkmark$  &  0.621&  0.857 &  0.304 &  110.0 \\
        \texttt{deepseek-v3}  &  $\checkmark$  &  0.691&  0.902 &  0.332 &  122.6 &  $\checkmark$  &  0.527 &  0.863 &  0.286 &  160.5 &  $\checkmark$  &  0.522&   0.851 &  0.275 &  113.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.673&  0.904 &  0.276 &  133.2 (1089.2) &  $\checkmark$  &  0.517 &  0.854 &  0.241 &  136.0 (972.7) &  $\checkmark$  &  0.554&  0.858 &  0.235 &  133.8 (611.1) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.673&  0.906 &  0.296 &  114.2 (1810.2) &  $\checkmark$  &  0.571 &  0.861 &  0.275 &  111.2 (2229.6) &  $\checkmark$  &  0.529&  0.855 &  0.256 &  110.8 (2158.8) \\

        \midrule
        \multicolumn{16}{l}{\textit{Category 4: Translate + Modify Pipeline (2 run)}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  0.694&  0.904 &  0.327 &  30.2 &  $\times$  &  0.653&  0.868 &  0.276 &  42.7 &  $\times$  &  0.643&  0.876 &  0.246 &  37.6 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.703&  0.934 &  0.322 &  88.1 &  $\times$  &  0.645&  0.874 &  0.239 &  89.4 &  $\times$  &  0.543& 0.873 &  0.221 &  102.1 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.691&  0.902 &  0.348 &  22.3 (2517.7) &  $\times$  &  0.627&  0.830 &  0.267 &  27.5 (1043.1) &  $\checkmark$  &  0.602&  0.840 &  0.250 &  22.4 (2975.2) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.690&  0.917 &  0.321 &  42.2 (2666.2) &  $\checkmark$  &  0.514&  0.842 &  0.275 &  46.6 (2773.0) &  $\checkmark$  &  0.557&  0.820 &  0.234 &  44.9 (4012.9) \\
        \midrule
        \multicolumn{16}{l}{\textit{Category 5: HOMURA}} \\
        \midrule
        \textbf{Ours (HOMURA\textsubscript{Rubric})}  &  $\checkmark$  &  0.700 &  0.914 &  0.378 &  9.2  & $\checkmark$  & 0.591 &   0.853 &  0.317 &  16.3&   $\checkmark$ &   0.620& 0.863 &  0.260 &  13.1\\
        \textbf{Ours (HOMURA\textsubscript{Reason})}  &  $\checkmark$  &  0.701 &  0.925 &  0.376 & 10.1& $\checkmark$  & 0.603 &   0.861 &  0.321  & 14.7&  $\checkmark$ &  0.605 &  0.858 &  0.309 &  13.2 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{2mm}
    
    \raggedright
    \footnotesize
    Note: IB: In Bounds, $\checkmark$ indicates within bounds, $\times$ indicates out of bounds. AVG-Tokens: Average number of output tokens per sample; for reasoning models ($^*$), values in parentheses denote the total tokens consumed (including internal thinking).

    \vspace{-4mm}
\end{table*}

\subsection{Experimental Setup}

% \subsubsection{Translation Strategies and Baselines}
We evaluate SOTA LLMs under five strategy categories that span the length-control spectrum:

\begin{itemize}[nosep]
    \item \textbf{Category 1: Unconstrained LLMs}. Frontier models (\texttt{GPT-5}~\cite{openai2025gpt5systemcard}, \texttt{Claude-4.1-Opus}~\cite{anthropic2025claude}, \texttt{Gemini-2.5-Pro}, \texttt{DeepSeek-V3}) with standard decoding. For \texttt{GPT-5} and \texttt{Gemini-2.5-Pro}, we set low reasoning effort to approximate direct translation. These serve as semantic upper bounds.
    \item \textbf{Category 2: Prompt-based Compression.} Category 1 models with brevity-oriented system prompts enforcing syllable-level conciseness.
    \item \textbf{Category 3: Best of N Refinement.} Generating $N$ candidates with varying lengths, followed by a greedy selection of the highest-fidelity output that fulfills the syllable budget.
    \item \textbf{Category 4: Pipeline-based Post-editing.} Two-stage translation $\rightarrow$ length-constrained rewriting.
    \item \textbf{Category 5: Our Method (HOMURA).} RL fine-tuning on \texttt{Qwen3-8B}~\citep{yang2025qwen3} to enforce temporal budgets as hard constraints.
\end{itemize}

More experimental details are provided in Appendix~\ref{sec:appendix_hyper}.

\subsection{Target Syllable Bounds Configuration}
\label{ssec:target_bounds}
Following Section~\ref{sec:verbosity_bias}, we set density-calibrated target bounds $\mathcal{B}_{L}$ to impose comparable compression pressure across languages: En $\in [0.8, 0.9]$, De $\in [0.9, 1.0]$, and Es $\in [1.0, 1.1]$. These intervals are used as hard constraints for HOMURA.

\subsubsection{Evaluation Metrics}
\label{sec:evaluation_metrics}
We report complementary metrics for efficiency, semantic preservation, and linguistic quality:

\paragraph{Translation Density (BLEU-$\rho$ $\uparrow$)}
We define \textbf{BLEU-$\rho$} as semantic fidelity per temporal unit:
\begin{equation}
    \text{BLEU-}\rho = \frac{\text{BLEU}(x, \hat{x})}{\rho(x,y)},
\end{equation}
where $\text{BLEU}(x,\hat{x})$ is the back-translation BLEU~\cite{papineni2002bleu}. Since BLEU alone may not fully capture fluency in back-translation paradigms~\cite{edunov-etal-2020-evaluation}, we use BLEU-$\rho$ specifically to measure \textbf{information density}, while linguistic quality assessed via Cometkiwi.

\paragraph{Semantic Integrity (BT-CERR $\uparrow$)}
BT-CERR is a binary indicator that evaluates whether all core events extracted from $x$ are retained in the back-translation $\hat{x}$.
 (see Appendix~\ref{sec:appendix_sand-glass_construction} for the definition of core events).
% BT-CERR verifies whether core predicates and essential arguments extracted from $x$ are retained in the back-translation $\hat{x}$.

\paragraph{Linguistic Quality (Cometkiwi $\uparrow$)}
We use reference-free Cometkiwi\cite{rei2022cometkiwi} to assess fluency and adequacy under compression.

\subsection{Main Results}
\label{sec:main_results}

\subsubsection{Cross-Lingual Performance and Temporal Compliance}
\label{sec:overall_performance}

Table~\ref{tab:main_results_cross_lingual} summarizes performance on Sand-Glass. We report human evaluation in Appendix~\ref{sec:appendix_human_judgment} and Statistical Significance Testing in Appendix~\ref{sec_statistical_test_appendix}. Overall, the results highlight the trade-off between temporal compliance and semantic density:

\paragraph{Budget Violation in Frontier Models.} 
As shown by the  IB column, unconstrained frontier model(\textsc{Cat 1}) universally fail to meet temporal budgets ($\times$), particularly in low-density languages like Spanish. While specialized prompting (\textsc{Cat 2}) shifts the distribution toward brevity, it remains unreliable, with models like \texttt{GPT-5} still exhibiting "verbosity drift" that exceeds target bounds. This confirms that pure instruction-following is insufficient for rigorous syllable-level constraints.

\paragraph{The Search-Fidelity Trade-off.} 
Search-based (\textsc{Cat 3}) and pipeline (\textsc{Cat 4}) strategies achieve higher In-Bounds rates but at a significant semantic cost. For instance, \textsc{Cat 4} variants often show a drop in BT-CERR, suggesting that the disjointed post-editing process leads to "hallucinated omissions" of critical source predicates. Moreover, the increased inference latency of Best-of-$N$ makes it less practical in real-time setting.

\begin{figure*}[th]
    \centering
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/bt_bleu_en_comparison.pdf}
        \caption{BLEU vs. Avg. Syllable Ratio}
        \label{fig:bt_bleu}
    \end{subfigure}\hfill
    \begin{subfigure}[t]{0.49\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/cerr_en_comparison.pdf}
        \caption{BT-CERR vs. Avg. Syllable Ratio}
        \label{fig:cerr_en}
    \end{subfigure}
    \caption{Quality--compression trade-off on \text{Zh}$\rightarrow$\text{En}. We plot BLEU (left) and BT-CERR (right) versus the average syllable ratio $\rho$. Each point is a model setting (marker: backbone; color: variant: Unconstrained, Rubric, GenRM, Multi-length Prompting). The red curve shows the empirical trend: quality degrades as compression strengthens.}
    
    \label{fig:tradeoff_curve}

    \vspace{-4mm}
\end{figure*}

\paragraph{Information Density Superiority of  HOMURA.} 
In contrast, HOMURA consistently maintains in bound while achieving the highest BLEU-$\rho$ across all language pairs. This gap demonstrates that HOMURA does not merely truncate text but actively performs \textit{semantic packing}—delivering a higher "semantic payload" per syllable. Additionally, we scale our method to a 32B model; see Appendix~\ref{sec:appendix_scale} for details.

\paragraph{Inference efficiency.}
HOMURA is markedly more inference-efficient. Unlike Best-of-$N$, which multiplies decoding cost by generating $N$ candidates, and unlike translate-then-modify pipelines that require an extra rewriting pass, HOMURA satisfies the syllable/temporal budget in a single decoding. Consequently, it attains high \textsc{IB} compliance with substantially fewer tokens (AVG-Tokens in Table~\ref{tab:main_results_cross_lingual}), making it suitable for real-time and high-throughput deployment.

\paragraph{Robustness of Reason-based GenRM.} 
Within Category~5, HOMURA\textsubscript{Reason} achieves higher BT-CERR than HOMURA\textsubscript{Rubric} on two of the three target languages, with the largest gain observed for English.
% Within Category~5, HOMURA\textsubscript{Reason} consistently achieves higher BT-CERR than HOMURA\textsubscript{Rubric}, with the largest gains on morphosyntactically complex targets (e.g., German). 
This suggests the reason-based reward better prunes redundancy while preserving the source’s logical structure. We further validate this by replacing the self-trained GenRM in HOMURA\textsubscript{Reason} with an LLM-as-RM baseline (\texttt{DeepSeek-V3}); results are in Appendix~\ref{sec_genrm_compare_appendix}.

\paragraph{Sensitivity of KL Regularization.}
While the theoretical objective in Eq.~\eqref{eq:kl-regularized-rl} assumes $\beta > 0$ for policy stability, our empirical investigations reveal a task-specific trade-off. 
As shown in our ablation experiments, introducing $\beta > 0$ leads to a notable degradation in structural alignment. 
This suggests that for time-constrained translation, the reference model $P_0$ imposes a ``verbosity prior'' that penalizes the radical lexical pruning and syntactic restructuring necessary to meet the Sand-Glass budget. 
By setting $\beta \to 0$ in our final implementation, we grant the model maximum \textit{compression freedom}. 
The inherent stability of the GRPO algorithm's group-relative optimization, coupled with the explicit guidance of our task-specific rewards, ensures that this relaxation preserves policy stability and prevents linguistic collapse, allowing HOMURA to reach a more efficient rate-distortion frontier. A detailed theoretical and empirical analysis of this stabilization mechanism is provided in Appendix \ref{app:stability_analysis}.

\subsubsection{Analysis of Quality--Compression Trade-off}
\label{sec:compression_tradeoff}

Figure~\ref{fig:tradeoff_curve} illustrates the trade-off between translation quality and output length. By plotting semantic metrics against the average syllable ratio $\rho$, we compare how different models perform as the available length budget decreases.

As shown in Figure~\ref{fig:tradeoff_curve}, unconstrained baselines cluster in the high-quality, high-$\rho$ region, representing the model's performance when length is not a factor. While standard LLMs can be prompted to shorten their outputs, their quality drops sharply as compression becomes more aggressive. This reflects a low rate--distortion efficiency: when forced to reduce the phonetic ``rate'' (syllables), these models suffer from disproportionately high ``distortion'' (loss of meaning), as they struggle to identify which information is most essential to preserve.

In contrast, HOMURA variants demonstrate significantly higher rate--distortion efficiency. At any given syllable budget, HOMURA maintains higher semantic fidelity than the baselines; conversely, it can achieve a much shorter length while maintaining the same quality level. These results suggest that our framework does not simply truncate text. Instead, it optimizes the model to operate at a more efficient trade-off point—packing a higher semantic payload into a limited phonetic budget to respect the strict constraints of media localization.
   
\iffalse
\subsubsection{Effect of GenRM Choice}
%\label{sec:ablation_studies}
%Table \ref{tab:ablation_study} compares HOMURA\textsubscript{Reason} with a variant that substitutes the self-trained GenRM with an external reward model implemented using DeepSeek-V3, a state-of-the-art general-purpose LLM. We report the average performance across all language pairs on three evaluation metrics.

As shown in the Table \ref{tab:ablation_study}, the compression translation model optimized with the self-trained GenRM consistently achieves better results than its counterpart using the external reward model. This indicates that a reward model trained to align with the specific objectives of compression-oriented translation provides more effective guidance during optimization. Consistent with this observation, on a held-out human-annotated reward model evaluation set designed to assess compression-aware translation quality, GenRM also demonstrates higher accuracy than the external RM, achieving 0.85 compared to 0.81. Details of the reward model evaluation set are provided in Appendix \ref{sec_genrm_test_appendix}.

\begin{table}[ht]
    \centering
    \caption{Effect of GenRM choice on compressed translation under HOMURA\textsubscript{Reason} (Average across all language pairs).}
    \label{tab:ablation_study}

    \footnotesize
    \setlength{\tabcolsep}{2.2pt}
    \renewcommand{\arraystretch}{0.95}

    \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccc}
        \toprule
        \textbf{Model Variant} & \textbf{BLEU-$\rho$} & \textbf{Cometkiwi} & \textbf{BT-CERR} \\
        \midrule
        HOMURA\textsubscript{Reason}  & 0.335 & 0.636 & 0.883 \\
        \midrule
        HOMURA\textsubscript{Reason} (w/ External RM)  & 0.330 &  0.628& 0.879 \\
        \bottomrule
    \end{tabular}%
    }
\end{table}
\fi

\subsubsection{Qualitative Case Studies}
\label{sec:case_studies}

We qualitatively compare HOMURA with representative baselines to assess practical behavior under different compression budgets.
As shown in Table~\ref{tab:combined_case_study}, frontier models (e.g., \texttt{GPT-5}, \texttt{Claude-4.1-opus}) often remain verbose even with brevity prompts, whereas HOMURA achieves tighter budget adherence by packing semantics into denser lexical and syntactic forms.
When the budget becomes extreme (down to $\rho \approx 0.25$), HOMURA smoothly shifts from natural prose to highly condensed translations, prioritizing core predicate--argument content while discarding redundant function words.
Full case comparisons and a taxonomy of the observed linguistic shifts are deferred to Appendix~\ref{sec:appendix_cases}.


% \subsubsection{Qualitative Case Studies}
% \label{sec:case_studies}

% To evaluate the practical efficacy of our framework, we conduct a qualitative analysis comparing HOMURA against representative baselines and examining its behavior across varying compression intensities.

% Table~\ref{tab:combined_case_study} in Appendix~\ref{sec:appendix_cases} presents a challenging \text{Zh}$\rightarrow$\text{En} instance that exemplifies the systemic \textit{verbosity bias} of frontier models. We observe that while models like \texttt{GPT-5} and \texttt{Claude-4.1} prioritize stylistic richness even with explicit prompting, HOMURA achieves precise adherence through active semantic packing. By mapping verbose syntactic structures to denser lexical equivalents (e.g., condensing a 7-syllable phrase into a 1-syllable noun), HOMURA demonstrates a superior ability to prioritize core information under strict temporal limits.

% Furthermore, our analysis of the model's tunability shows a graceful transition from natural prose to highly condensed strategies as the budget $\rho$ approaches the empirical compression limit ($\rho \approx 0.25$). In this extreme regime, HOMURA strategically prioritizes predicate-argument structures over functional redundancy, effectively navigating the trade-off between linguistic richness and feasibility. A detailed taxonomic breakdown of these linguistic shifts and the full case comparison are provided in Appendix~\ref{sec:appendix_cases}.



\subsection{Autonomous Compression: Navigating the Compression Limit}
\label{sec:auto_compression}

The preceding experiments show that HOMURA can reliably translate under a user-specified ratio interval. We further ask whether, without a preset lower bound, the model can \emph{autonomously} discover the practical compression limit: the point where additional shortening triggers a sharp loss in meaning. To this end, we formulate an autonomous compression task by replacing the hard-interval length reward with a continuous incentive:
\begin{align}
R_{\mathrm{len}}^{\mathrm{(auto)}}(x, y) = \min\left(\cos\left(\theta \cdot \rho(x, y)\right),\; 0\right),
\end{align}
where $\theta$ scales the incentive gradient. The policy is encouraged to minimize $\rho$ while still being constrained by the quality reward $R_{\mathrm{qual}}$.

\begin{table}[t] 
\centering 
\caption{The Compression Wall. The autonomous model reliably reaches the feasible limit; stricter manual targets miss $\rho$ and produce worse compression.}
\label{tab:auto_compression_results} 
\scriptsize 
\setlength{\tabcolsep}{10pt}
\begin{tabular}{lccc} \toprule 
\textbf{Model \& Configuration} & $\boldsymbol{\rho}$ & \textbf{BLEU-$\boldsymbol{\rho}$} & \textbf{BT-CERR}\\ 
\midrule \textbf{Auto HOMURA} & \textbf{0.485} & 0.404 & 0.811 \\ 
% \textbf{Auto HOMURA\textsubscript{Reason}} & \textbf{0.459} & 0.390 & 0.805\\ 
\midrule \multicolumn{4}{l}{\textit{Manually Constrained HOMURA}} \\ 
\hspace{1mm} $R_{\mathrm{target}} \in [0.3, 0.4]$ & 0.558 & 0.392 & 0.819\\
\hspace{1mm} $R_{\mathrm{target}} \in [0.4, 0.5]$ & \textbf{0.481} & 0.384 & 0.816\\ 
\hspace{1mm} $R_{\mathrm{target}} \in [0.5, 0.6]$ & 0.559 & 0.386 & 0.856\\
\hspace{1mm} $R_{\mathrm{target}} \in [0.8, 0.9]$ & 0.808 & 0.378 & 0.914\\ 
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

% \paragraph{The Empirical Compression Wall}

% A consistent \textit{compression wall} emerges when the model is pushed toward its structural limits. As shown in Table~\ref{tab:auto_compression_results}, when optimized autonomously, the model converges to a stable average ratio of $\rho \approx 0.485$. 

% Notably, even when we impose an \textit{ultra-aggressive target bound} of $[0.3, 0.4]$---a range that likely exceeds the theoretical limit of information density---the model fails to reach shorter lengths. Instead, the achieved ratio regresses to $\rho=0.558$, accompanied by a severe drop in semantic coherence. This non-linear response suggests that $\rho \approx 0.49$ represents a \textit{critical feasibility threshold} for Zh-to-En translation. Any attempt to compress beyond this ``wall'' triggers a conflict between length and quality rewards, where the model can no longer maintain basic syntax while staying brief.

\paragraph{The Empirical Compression Wall}

We observe a stable \textit{compression wall} when pushing the model to its structural limit. In Table~\ref{tab:auto_compression_results}, autonomous optimization consistently converges to a narrow operating regime around $\rho \in [0.46, 0.49]$, regardless of the specific reward configuration.

When we enforce an ultra-aggressive target of $[0.3, 0.4]$, the model does \emph{not} become shorter; instead it rebounds to $\rho=0.558$ and semantic coherence collapses. This non-linear failure indicates a feasibility threshold around $\rho \approx 0.49$ for Zh$\rightarrow$En: compressing beyond it creates an irreconcilable length-quality trade-off, where the model cannot preserve basic well-formedness while remaining brief.

\paragraph{Efficiency at the Frontier}
To quantify compression efficiency, we report BLEU-$\rho$. The autonomous model attains the best BLEU-$\rho$ while operating at a genuinely shorter length ($\rho=0.485$ vs.\ $0.558$), indicating that autonomous optimization finds a more efficient operating point on the quality-compression frontier.

\paragraph{Rate-Distortion Efficiency at the Frontier}
Qualitatively, the autonomous model tends to compress by \emph{semantic condensation}: dropping modifiers, selecting denser lexical items, and simplifying clause structures. In contrast, when forced toward an overly aggressive interval, outputs more often exhibit unstable shortening behaviors, reflecting the tension between further length reduction and preserving core meaning.

\paragraph{Takeaway: The Wall as a Feasibility Boundary}
Together, these results suggest an empirical feasibility boundary around $\rho\approx0.49$ for time-constrained translation in our setting (Zh→En).% This empirical limit closely aligns with the theoretical density floor predicted by the Iso-Information Principle introduced in Section \ref{sec:verbosity_bias}.
We hypothesize that this boundary represents the minimal information carrier required to express core predicate-argument content.


==> section_backup_old/IntroductionV2.tex <==
\section{Introduction}

With the rapid advancement of Large Language Models (LLMs), their multilingual capabilities have achieved unprecedented semantic adequacy and fluency in Neural Machine Translation (NMT)~\cite{hendy2023good, jiao2023chatgpt, zhu2024multilingual}. However, this linguistic prowess is accompanied by a systemic cross-lingual verbosity bias~\cite{briakou2024implications, manakhimova2024investigating}. As illustrated in Figure~\ref{fig:roundtrip_case}, LLM-generated translations tend to be significantly longer than their source utterances, a "chattiness" that persists even when semantic content remains constant. While acceptable in general text generation, this expansion becomes a critical failure mode in time-constrained scenarios such as subtitles, video dubbing, and simultaneous interpretation,where translation length constitutes a rigid temporal budget that strictly limits the output duration~\cite{karakanta-etal-2020-must, jorgensen-mengshoel-2025-cross, gaido2024automatic}.
To operationalize the temporal budget, we approximate the available speaking time with a cross-lingually comparable syllable budget.

\begin{figure}[t]
\centering
  \includegraphics[width=\linewidth]{images/roundtrip-case.pdf}
\caption{Illustration of cross-lingual verbosity bias. Unlike forward metrics, the \textbf{Roundtrip Expansion Ratio} $\rho_{\text{rtp}}$ isolates model-induced redundancy from linguistic density shifts. A value of $\rho_{\text{rtp}} > 1.0$ indicates systemic inflation despite constant semantic content. Formal definition and diagnostic study are provided in Section~\ref{sec:pilot}.}
 \label{fig:roundtrip_case}
\end{figure}

Viewed through an information-theoretic lens ~\cite{shannon1948mathematical, davisson1972rate}, these temporal budgets act as a strict rate constraint: with a limited number of target syllables available, the model must pack maximal meaning into minimal length, implicitly operating near a rate-distortion limit on the achievable fidelity compression trade-off. In our setting, the rate is the syllable budget, and distortion can be understood as the loss in meaning or adequacy relative. 
% Viewed through an information-theoretic lens, time-constrained translation imposes a strict rate constraint: the output must fit within a fixed syllable budget.
% This inevitably introduces a fidelity--compression trade-off: compress too much and meaning is lost; exceed the budget and synchronization breaks.
Unfortunately, off-the-shelf LLMs struggle to respect these limits. This failure is deeply rooted in the post-training alignment process, where learned reward models frequently exhibit a "length bias" that conflates verbosity with quality~\cite{saito2023verbosity, singhal2023long}. 
Furthermore, cross-lingual typological differences systematically skew length ratios, transforming length control from a superficial formatting task into a first-class modeling challenge.
\footnote{Detailed related works can be found in appendix \ref{sec:appendix_related_works}.}

To address this fundamental mismatch between LLM capabilities and temporal constraints, we argue that length control should be treated as an optimization objective rather than a post-hoc adjustment. To this end, we first operationalize the problem by constructing \emph{Sand-Glass}, a dedicated benchmark for time-constrained media localization. The name reflects the rigid temporal budget that "drains" as the model produces redundant tokens. 
Unlike generic translation datasets, Sand-Glass incorporates syllable-based duration proxies calibrated by Information Density (ID), derived from real-world colloquial subtitles enabling precise evaluation of length compliance.

Building on this testbed, we propose \emph{HOMURA} (\textbf{H}ard \textbf{O}ptimization for \textbf{M}ultilingual \textbf{U}tterance \textbf{R}eduction and \textbf{A}lignment), a reinforcement learning framework designed to ``tame the sandglass'' by explicitly regulating translation length without requiring supervised compression datasets. Instead of relying on brittle prompts, HOMURA optimizes the quality compression trade-off directly. We design a novel reference free reward function that combines a dynamic syllable ratio penalty with a semantic fidelity reward, encouraging the model to condense information density without sacrificing core meaning.

Our core contributions are as follows:
\begin{itemize}[nosep]
    \item \textbf{Diagnostic Analysis:} We systematically quantify the verbosity bias in LLM-based translation under temporal constraints, providing cross-lingual diagnostics (e.g., the $\rho_{\text{rtp}}$ metric) that reveal the limitations of unconstrained models as visualized in Figure~\ref{fig:roundtrip_case}.
    \item \textbf{Benchmark Construction:} We introduce Sand-Glass, a specialized dataset tailored for time-constrained translation, featuring syllable-level duration budgets to simulate real-world dubbing and subtitling scenarios.
    \item \textbf{Methodological Innovation:} We propose HOMURA, a KL-regularized RL framework that dynamically balances strict length constraints with semantic preservation, significantly outperforming strong LLM baselines in both compliance and quality.
\end{itemize}

==> section_backup_old/Method.tex <==
\section{Method}

We formulate syllable-level control as a standard controllable text generation task\cite{li2024reinforcement, gu2025length}, where our objective is to maximize translation quality while satisfying the prescribed syllable-ratio constraint. Our method is illustrated in Figure \ref{fig:method}.


\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{images/method4.pdf}
\caption{Overview of our HOMURA framework. Given a source utterance $x$ and a syllable-ratio budget $c$, we optimize a KL-regularized policy $\pi_\theta(y\!\mid\!x,c)$ with GRPO. The reward combines a length-compliance term $R_{\mathrm{len}}$ and a quality term $R_{\mathrm{qual}}$ (rubric-based or reason-based), encouraging concise yet faithful translations.}
\label{fig:method}
\vspace{-2mm}
\end{figure*}

\subsection{KL-Regularized Objective for Controllable Generation}

We study conditional generation with an input $x$ and a control condition $c$. Our objective is to learn a policy $\pi_\theta(y\mid x,c)$ that satisfies $c$.

\paragraph{Target Distribution via a Controlled Posterior.}
A natural target distribution for controllable generation is the controlled posterior
\begin{equation}
P(y \mid x,c) \propto P(c \mid x,y)\, P_0(y \mid x),
\label{eq:controlled-posterior}
\end{equation}
where $P(c\mid x,y)$ measures how well an output $y$ meets the control condition, and $P_0(y\mid x)$ denotes a fixed reference model that captures the unconstrained translation distribution given the input $x$.

\paragraph{KL Projection.}
We fit $\pi_\theta(\cdot\mid x,c)$ by projecting it onto the target distribution:
\begin{equation}
\pi_\theta^\star(\cdot\mid x,c)
=\arg\min_{\pi_\theta}\ \mathrm{KL}\!\left(\pi_\theta(\cdot\mid x,c)\ \|\ P(\cdot\mid x,c)\right).
\label{eq:kl-proj}
\end{equation}
Ignoring constants independent of $\theta$ and using Eq.~\eqref{eq:controlled-posterior}, this objective is equivalent to maximizing
\begin{align}
J(\theta)
&= \mathbb{E}_{y\sim \pi_\theta}
\Big[
\log P(c\mid x,y)
-\beta \log \tfrac{\pi_\theta(y\mid x,c)}{P_0(y\mid x)}
\Big],
\label{eq:kl-regularized-rl}
\end{align}
where $\beta>0$ is a temperature (or weighting) coefficient that controls the strength of KL regularization.
In practice, we model $\log P(c\mid x,y)$ with a task reward $R(x,c,y)$.

Eq.~\eqref{eq:kl-regularized-rl} can be viewed as a KL-regularized reinforcement learning objective:
$R(x,c,y)$ encourages satisfying the control condition, while the KL term discourages drifting away from the base model $P_0$.
The coefficient $\beta$ controls the trade-off between control strength and faithfulness.


\paragraph{Optimization with GRPO.}
We optimize Eq.~\eqref{eq:kl-regularized-rl} using GRPO \citep{shao2024deepseekmath}, a lightweight PPO-style
algorithm for sequence-level rewards. For each $(x,c)$, we sample multiple
candidates from the previous policy $\pi_{\theta_{\text{old}}}$, compute rewards
and group-normalized advantages, and update $\pi_\theta$ with a clipped policy
objective together with the KL regularization toward $P_0$.

\subsection{Reward Design}
\label{sec:reward}
In our setting, the control condition $c$ corresponds to satisfying a strict length budget while maintaining semantic consistency with the source. This requires a reward that simultaneously encourages length compliance and discourages meaning drift. 
% Therefore, we instantiate the generic controllable reward $R(x,c,y)$ in Eq.~\eqref{eq:kl-regularized-rl} as a weighted sum of two complementary terms:
We interpret $\log P(c\mid x,y)$ in Eq.~\eqref{eq:kl-regularized-rl} as a task reward, denoted by $R(x,c,y)$, and instantiate it as:
\begin{align}
R(x,c,y)
= \lambda_{\mathrm{len}} \, R_{\mathrm{len}}(x,y)
+ \lambda_{\mathrm{qual}} \, R_{\mathrm{qual}}(x,y),
\end{align}
where $x$ is the source utterance, $y$ is the generated translation, and $\lambda_{\mathrm{len}}, \lambda_{\mathrm{qual}} \ge 0$ control the trade-off between temporal alignment and semantic fidelity.

\subsubsection{Dynamic Syllable-ratio Reward}
\label{sec:dynamic_reward}

To ensure the translation length aligns naturally with the source speech across varying scales, we propose a dynamic syllable-ratio reward. The syllable ratio $\rho$ for a source-target pair $(x, y)$ is defined as:
\begin{equation}
\rho(x,y) = \frac{\sigma(y)}{\max(\sigma(x), 1)},
\end{equation}
where $\sigma(\cdot)$ is the syllable count of a sequence.

Recognizing that strict length constraints must be sensitive to both linguistic density and utterance length, we implement a dynamic acceptance interval $[L(x), R(x)]$. We initialize the baseline bounds $[L_0, R_0]$ using the language-specific Target Bounds $\mathcal{B}_L$ set in Section~\ref{sec:verbosity_bias}. This ensures the optimization target respects the cross-lingual density hierarchy established in our theoretical analysis.

However, for shorter utterances, the ``granularity'' of syllable counting introduces high variance (discretization noise), making rigid bounds brittle. To address this, for utterances where the source length $\sigma(x)$ is below the corpus mean $\mu$, we define a scaling factor $\gamma(x)$ to adaptively relax the lower threshold:
\begin{equation}
\gamma(x) = \alpha_1 + \alpha_2 \left( \frac{\sigma(x)}{\mu} \right)^{1/2},
\end{equation}
where $\alpha_1, \alpha_2$ are hyperparameters governing the degree of relaxation. The final dynamic bounds are formulated as $[L(x), R(x)] = [L_0 \cdot \gamma(x), \, R_0]$.

To facilitate stable policy optimization, we avoid sparse or binary signals in favor of a smoother reward landscape. The reward function $R_{\mathrm{len}}(x,y)$ evaluates compliance with these dynamic boundaries via a squared exponential decay:
\begin{equation}
R_{\mathrm{\rho}} = 
\begin{cases} 
1 & \text{if } \rho \in [L(x), R(x)] \\
\exp(-k \delta^2) & \text{otherwise}
\end{cases}
\end{equation}
where $\delta(x,y) = \max\bigl(|\rho(x,y) - L(x)|, |\rho(x,y) - R(x)|\bigr)$ denotes the deviation. This non-linear formulation provides a soft penalty that effectively guides the model toward the density-calibrated region while preventing training instability associated with hard-truncation rewards. In Appendix~\ref{sec:appendix_dynamic_reward}, we further investigate the effectiveness of a static syllable-ratio reward.


\subsubsection{Rubric-based Quality Reward}
We adopt a two-part quality rubric\cite{hashemi2024llm, liu2023g}, covering (i) semantic fidelity and (ii) linguistic well-formedness, and implement it as the following reward components.

\paragraph{Semantic Fidelity Reward}
\label{sec:sem_reward}

Inspired by the probabilistic duality in \citep{he2016dual}, we enforce content preservation via a reconstruction-based reward. We employ a frozen \texttt{DeepSeek-V3} \citep{deepseekai2024deepseekv3technicalreport} to back-translate the hypothesis $y$ into $\hat{x} = f_{bt}(y)$. To measure semantic retention, we compute the cosine similarity $S(x, \hat{x})$ between embeddings of the source $x$ and reconstruction $\hat{x}$ extracted by \texttt{Qwen-Embedding-0.6B} \citep{qwen3embedding}:

\begin{equation}
    S(x, \hat{x}) = \frac{\mathbf{v}_x \cdot \mathbf{v}_{\hat{x}}}{\|\mathbf{v}_x\| \|\mathbf{v}_{\hat{x}}\|}
\end{equation}

The final reward is clipped to stabilize optimization:
\begin{equation}
    R_{bt}(x, y) = \text{clip}(S(x, \hat{x}), \tau_{min}, \tau_{max})
\end{equation}

\paragraph{Linguistic Well-formedness Reward}
\label{sec:ling_reward}

To prevent the telegraphic outputs often associated with aggressive compression, we explicitly penalize linguistic degradation. We utilize a frozen \texttt{DeepSeek-V3} as a judge to evaluate translations against a rubric covering: (i) \textit{grammaticality}, (ii) \textit{readability}, and (iii) \textit{language consistency} (e.g., no code-switching). The model outputs a binary decision $s_{flu} \in \{0, 1\}$, serving directly as the reward:

\begin{equation}
    R_{flu}(x, y) = s_{flu}
\end{equation}

Full prompting details are in Appendix~\ref{sec:prompt_fluency}.

% \paragraph{Complementarity of the two rewards.}
% Together, $R_{\mathrm{bt}}$ and $R_{\mathrm{flu}}$ are designed to ensure that compression does not come at the cost of quality:
% $R_{\mathrm{bt}}$ emphasizes preserving the source content (completeness/fidelity), while $R_{\mathrm{flu}}$ emphasizes producing fluent and grammatical target sentences.

\subsubsection{Reason-based Quality Reward}
Beyond the simple compositional rewards, we explore an end-to-end generative reward model (GenRM)\cite{mahan2024generative, liang2025generative} that evaluates translation quality via explicit reasoning.
GenRM is trained using structured Chain-of-Thought (CoT) annotations synthesized by \texttt{Gemini-2.5-Pro} \citep{comanici2025gemini}. To ensure high-quality reasoning, we filter the raw CoT data using the aforementioned rubric-based method. The model is instantiated from \texttt{Qwen3-32B}~\citep{yang2025qwen3} and optimized via supervised fine-tuning (SFT) over the full CoT sequence and the final decision token.

Given a source sentence $x$ and a translation hypothesis $y$, GenRM performs a single long CoT reasoning process that can be abstracted as
\begin{equation}
\hat{x} = f_{\mathrm{bt}}(y),\;
s(x, \hat{x}), q(y) \in \{0,1\},
\end{equation}
where $f_{\mathrm{bt}}$ denotes implicit back-translation, $s(x, \hat{x})$ indicates whether the core information in $x$ is preserved, and $q(y)$ evaluates the intrinsic quality of $y$ in terms of adequacy and fluency. Based on these decisions, GenRM outputs a binary quality reward
\begin{equation}
R_{gen}(x,y) = \mathbb{I}\big[s(x,\hat{x}) =1 \land q(y)=1\big].
\end{equation}
This formulation yields a reference-free, interpretable quality signal and enforces an explicit conjunction between information preservation and translation quality. Concrete examples of the CoT reasoning are provided in the Appendix \ref{sec_genrm_example_appendix}.

% genRM is trained by us to perform translation quality evaluation via a structured long chain-of-thought (CoT) reasoning process. Rather than producing a continuous similarity score, genRM is trained to make discrete quality judgments based on explicit multi-step reasoning.
% Given a source sentence $x$ and a translation hypothesis $y$, genRM conducts a three-step reasoning procedure within a single long CoT.
% \begin{itemize}
%     \item First, the model generates a back-translation $\hat{x}$ from $y$.
%     \item Second, it evaluates the semantic similarity between $\hat{x}$ and the original source $x$, determining whether the core information is preserved.
%     \item Third, conditioned on sufficient semantic similarity, the model assesses the intrinsic quality of the translation $y$, focusing on adequacy and fluency.
% \end{itemize}

% Based on the outcome of this reasoning process, genRM outputs a binary quality reward:
% \begin{equation}
% R_{gen}(x,y) = \mathbb{I}\big[s(x,\hat{x}) =1 \land q(y)=1\big].
% \end{equation}
% A positive reward is assigned only when both information preservation and translation quality criteria are satisfied, enforcing an explicit conjunction between adequacy and compression.

% Compared to the compositional rewards, GenRM provides a reasoning-driven and interpretable quality signal while remaining reference-free.
% The two quality rewards reflect different inductive biases for quality estimation, and we evaluate both formulations in our experiments.


==> section_backup_old/Pilot_Experiment_Analysis.tex <==
\section{Pilot Study: Benchmark and Verbosity Bias}
\label{sec:pilot}

\begin{figure*}[th]
\centering
\includegraphics[width=0.95\textwidth]{images/3_scatter_forward_vs_backward.pdf}
\vspace{-2mm}
\caption{Forward vs.\ backward expansion relationship (colored by round-trip ratio $\rho_{\text{rtp}}$). The red curve represents the unity baseline $\rho_{\text{rtp}}=1.0$ ($y=1/x$). Points above this curve indicate systemic model-induced length inflation. Unconstrained models show a median $\rho_{\text{rtp}} > 1.10$.}
\label{fig:scatter_forward_backward}
\vspace{-3mm}
\end{figure*}

\subsection{The Sand-Glass Benchmark}
To diagnose cross-lingual verbosity bias under temporal constraints, we introduce Sand-Glass, a benchmark derived from colloquial video transcripts. Unlike generic datasets, it incorporates syllable-based duration proxies to strictly test time-sensitive compliance. The construction involves duration-aware segmentation based on speech pauses and core event extraction for semantic evaluation. We refer readers to Appendix \ref{sec:appendix_sand-glass_construction} for detailed protocols on dataset filtering and event extraction.

\subsection{Syllable as Duration Proxy}
\label{sec:syllable_proxy}
Our use of syllables as duration proxies is grounded in the Iso-Information Principle. Pellegrino \cite{Pellegrino2011language} demonstrated that while Syllable Rate (SR) vary drastically across languages (e.g., Spanish $7.82 \sigma/s$ [syllables/s] vs.\ Mandarin $5.18 \sigma/s$), the universal Information Rate remains nearly constant at $\approx 39$ bits/s~\cite{Coupe2019efficiency}.Recent findings further corroborate this by quantifying a universal surprisal–duration trade-off \citep{pimentel-etal-2021-surprisal}, showing that languages systematically adjust segment duration to smooth information transmission.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{3pt}
\begin{tabular}{lccc}
\toprule
\textbf{Language} & \textbf{Syllable Rate} & \textbf{Info. Density} & \textbf{Expansion} \\
& ($\sigma/s$) & (Normalized) & (from Zh) \\
\midrule
Mandarin (Zh) & $5.18 \pm 0.15$ & $0.94$ & $1.00\times$ \\
English (En) & $6.19 \pm 0.16$ & $0.91$ & $\approx 1.03\times$ \\
German (De) & $5.97 \pm 0.19$ & $0.79$ & $\approx 1.19\times$ \\
Spanish (Es) & $7.82 \pm 0.16$ & $0.63$ & $\approx 1.49\times$ \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Cross-linguistic statistics adapted from Pellegrino \cite{Pellegrino2011language}. Lower density necessitates higher expansion factors when translating from Mandarin.}
\label{tab:density_stats}
\vspace{-3mm}
\end{table}

As shown in Table~\ref{tab:density_stats}, this trade-off implies that low-density languages must utilize higher syllable counts to convey equivalent content. Translating from a high-density source (Mandarin, ID=0.94) to a lower-density target (e.g., Spanish, ID=0.63) necessitates a \textit{linguistically required expansion}. A direct 1:1 mapping would result in $\approx 33\%$ information loss (derived from the density ratio $\frac{0.63}{0.94}$). Thus, our constraints are non-uniform and calibrated to these density ratios to distinguish legitimate expansion from model verbosity.




\subsection{Quantifying Cross-Lingual Verbosity Bias}
\label{sec:verbosity_bias}

Standard metrics like the Forward Expansion Ratio defined as $\rho_{fwd} = \sigma(y)/\sigma(x)$ for a source $x$ and its translation $y$ often confound \textit{linguistic necessity} with \textit{model hallucinations}. For instance, a high $\rho_{fwd}$ in Spanish might simply reflect its naturally lower information density rather than model-induced redundancy. 

To isolate systemic bias, we introduce the \textit{Roundtrip Expansion Ratio} ($\rho_{rtp}$). By translating the target output $y$ back into the source language ($\hat{x}$) and comparing its syllable count to the original input $x$, we define:
\begin{equation}
    \rho_{rtp} = \rho_{fwd} \cdot \rho_{bwd} = \frac{\sigma(y)}{\sigma(x)} \cdot \frac{\sigma(\hat{x})}{\sigma(y)} = \frac{\sigma(\hat{x})}{\sigma(x)},
\end{equation}
where $\sigma(\cdot)$ denotes the syllable count of a sequence. Theoretically, since this comparison is performed within the same source language, $\rho_{rtp}$ should gravitate towards 1.0. Any value where $\rho_{rtp} > 1.0$ serves as a density-invariant indicator of model-induced inflation. 



Empirical analysis on Sand-Glass (Figure~\ref{fig:scatter_forward_backward}) confirms that this verbosity is systemic rather than anecdotal. By plotting the joint distribution of expansion ratios, we observe a pervasive upward shift from the unity baseline ($\rho_{rtp}=1.0$), with the vast majority of segments clustered in the ``inflation zone.'' This concentration demonstrates a consistent model-induced redundancy that persists across various frontier models and language pairs (see Appendix~\ref{sec:appendix_noraml_roundtrip_metrics} for statistical breakdowns).

\paragraph{Calibrated Target Bounds.}
To bridge this gap, we define Target Syllable Bounds ($\mathcal{B}_{L}$) by contrasting model inflation ($\mu_{LLM}$) against Theoretical Expansion ($\mu_{theo}$). As shown in Table~\ref{tab:expansion_comparison}, LLMs produce significant surplus bias ($\Delta_{bias}$). We establish $\mathcal{B}_{L}$ to enforce a strict condensation regime. Notably, we lower these targets beyond theoretical baselines to address real-world dubbing and subtitling complexities, specifically to buffer against rapid speech and synchronization constraints. Accordingly, we configure the bounds as follows:
English ($\mathcal{B}_{En}\in[0.8, 0.9]$) is set below parity to force active summarization;
German ($\mathcal{B}_{De}\in[0.9, 1.0]$) maintains relative pressure despite lower density;
and Spanish ($\mathcal{B}_{Es}\in[1.0, 1.1]$) significantly reduces the unconstrained baseline of $1.84\times$ to ensure intelligibility under strict time limits while respecting its information density.

\begin{table}[t]
\centering
\small
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lccc|c}
\toprule
\textbf{Target} & \textbf{Theoretical} & \textbf{LLM Baseline} & \textbf{Bias} & \textbf{Ours (Target)} \\
\textbf{Lang} & ($\mu_{theo}$) & ($\mu_{LLM}$) & ($\Delta$) & ($\mathcal{B}_L$) \\
\midrule
En & $1.03\times$ & $1.35\times$ & $+0.32$ & $\mathbf{0.8} \sim \mathbf{0.9}$ \\
De & $1.19\times$ & $1.59\times$ & $+0.40$ & $\mathbf{0.9} \sim \mathbf{1.0}$ \\
Es & $1.49\times$ & $1.84\times$ & $+0.35$ & $\mathbf{1.0} \sim \mathbf{1.1}$ \\
\bottomrule
\end{tabular}
\vspace{-2mm}
\caption{Comparison of expansion ratios. Target Bounds ($\mathcal{B}_L$) are set to remove model bias ($\Delta$) and enforce semantic condensation.}
\label{tab:expansion_comparison}
\vspace{-3mm}
\end{table}



==> test.tex <==
\section{Experiments and Results}
\label{sec_experiment}

\begin{table*}[t]
    \centering
    \caption{Performance Comparison on Sand-Glass Across All Language Pairs ($\text{BLEU-$\rho$}$, $\text{Cometkiwi}$, $\text{BT-CERR}$).  All results are averaged by 3 times.}
    \label{tab:main_results_cross_lingual}
    
    \Large
    \setlength{\tabcolsep}{5pt}
    \renewcommand{\arraystretch}{1.1}

    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|cccccc|cccccc|cccccc}
        \toprule
        \multirow{3}{*}{\textbf{Model}} & \multicolumn{18}{c}{\textbf{Evaluation Metrics on Sand-Glass}} \\
        \cmidrule(lr){2-19}
         & \multicolumn{6}{c|}{\textbf{Zh $\rightarrow$ En}} & \multicolumn{6}{c|}{\textbf{Zh $\rightarrow$ De}} & \multicolumn{6}{c}{\textbf{Zh $\rightarrow$ Es}} \\
        \cmidrule(lr){2-7} \cmidrule(lr){8-13} \cmidrule(lr){14-19}
          &  \textbf{IB}  &  \textbf{$\rho$}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{$\rho$}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens}  &  \textbf{IB}  &  \textbf{$\rho$}  &  \textbf{Cometkiwi}  &  \textbf{BT-CERR}  &  \textbf{BLEU-$\rho$}  &  \textbf{AVG-Tokens} \\
        \midrule
        \multicolumn{19}{l}{\textit{Category 1: w/o Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  1.148  &  0.741  &  0.943 &  0.313 &  17.1 &  $\times$  &  1.328  &  0.676&  0.882 &  0.247 &  24.2 &  $\times$  &  1.531  &  0.668&  0.900 &  0.220 &  21.3 \\
        \texttt{deepseek-v3}  &  $\times$  &  1.197  &  0.748  &  0.941 &  0.287 &  46.3 &  $\times$  &  1.408  &  0.676&  0.889 &  0.222 &  62.3 &  $\times$  &  1.653  &  0.671&  0.884 &  0.191 &  99.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  1.084  &  0.739  &  0.941 &  0.307 &  12.1 (916.9) &  $\times$  &  1.268  &  0.666&  0.877 &  0.238 &  14.2 (125.8) &  $\times$  &  1.452  &  0.668&  0.883 &  0.212 &  14.0 (1532.7) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  1.112  &  0.746  &  0.947 &  0.300 &  22.4 (412.8) &  $\times$  &  1.365  &  0.681&  0.894 &  0.220 &  23.2 (605.6) &  $\times$  &  1.556  &  0.671&  0.899 &  0.206 &  24.0 (676.8) \\

        \midrule
        \multicolumn{19}{l}{\textit{Category 2: w/ Syllable Constraint}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.852  &  0.691&  0.907 &  0.376&  12.2 &  $\checkmark$  &  0.951  &  0.535 &  0.838 &  0.293 &  17.2 &  $\times$  &  1.106  &  0.631&  0.849 &  0.261 &  13.5 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.960  &  0.700&  0.924 &  0.307 &  12.4 &  $\times$  &  1.196  &  0.557 &  0.866 &  0.245 &  15.8 &  $\times$  &  1.355  &  0.556 &  0.868 &  0.225 &  16.3 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\times$  &  0.920  &  0.698&  0.927 &  0.322 &  10.7 (1231.3) &  $\times$  &  1.016  &  0.517 &  0.853 &  0.266 &  12.3 (1450.1) &  $\times$  &  0.974  &  0.586&  0.827 &  0.252 &  10.7 (554.5) \\
        \texttt{gpt-5}$^*$  &  $\times$  &  0.937  &  0.705&  0.928 &  0.345 &  21.7 (2024.9) &  $\times$  &  1.025  &  0.534 &  0.874 &  0.283 &  23.1 (1962.3) &  $\times$  &  0.982  &  0.586&  0.833 &  0.270 &  21.0 (3105.8) \\

        \midrule
        \multicolumn{19}{l}{\textit{Category 3: Best of N}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\checkmark$  &  0.845  &  0.691&  0.903 &  0.367 &  109.7 &  $\checkmark$  &  0.946  &  0.611 &  0.848 &  0.324 &  109.2 &  $\checkmark$  &  1.039  &  0.621&  0.857 &  0.304 &  110.0 \\
        \texttt{deepseek-v3}  &  $\checkmark$  &  0.852  &  0.691&  0.902 &  0.332 &  122.6 &  $\checkmark$  &  0.959  &  0.527 &  0.863 &  0.286 &  160.5 &  $\checkmark$  &  1.042  &  0.522&   0.851 &  0.275 &  113.6 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.900  &  0.673&  0.904 &  0.276 &  133.2 (1089.2) &  $\checkmark$  &  0.992  &  0.517 &  0.854 &  0.241 &  136.0 (972.7) &  $\checkmark$  &  1.087  &  0.554&  0.858 &  0.235 &  133.8 (611.1) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.888  &  0.673&  0.906 &  0.296 &  114.2 (1810.2) &  $\checkmark$  &  0.994  &  0.571 &  0.861 &  0.275 &  111.2 (2229.6) &  $\checkmark$  &  1.076  &  0.529&  0.855 &  0.256 &  110.8 (2158.8) \\

        \midrule
        \multicolumn{19}{l}{\textit{Category 4: Translate + Modify Pipeline (2 run)}} \\
        \midrule
        \texttt{claude-4.1-opus}  &  $\times$  &  0.918  &  0.694&  0.904 &  0.327 &  30.2 &  $\times$  &  1.089  &  0.653&  0.868 &  0.276 &  42.7 &  $\times$  &  1.284  &  0.643&  0.876 &  0.246 &  37.6 \\
        \texttt{deepseek-v3}  &  $\times$  &  0.967  &  0.703&  0.934 &  0.322 &  88.1 &  $\times$  &  1.154  &  0.645&  0.874 &  0.239 &  89.4 &  $\times$  &  1.301  &  0.543& 0.873 &  0.221 &  102.1 \\
        \texttt{gemini-2.5-pro}$^*$  &  $\checkmark$  &  0.837  &  0.691&  0.902 &  0.348 &  22.3 (2517.7) &  $\times$  &  1.001  &  0.627&  0.830 &  0.267 &  27.5 (1043.1) &  $\checkmark$  &  1.042  &  0.602&  0.840 &  0.250 &  22.4 (2975.2) \\
        \texttt{gpt-5}$^*$  &  $\checkmark$  &  0.833  &  0.690&  0.917 &  0.321 &  42.2 (2666.2) &  $\checkmark$  &  0.934  &  0.514&  0.842 &  0.275 &  46.6 (2773.0) &  $\checkmark$  &  1.018  &  0.557&  0.820 &  0.234 &  44.9 (4012.9) \\
        \midrule
        \multicolumn{19}{l}{\textit{Category 5: HOMURA}} \\
        \midrule
        \textbf{Ours (HOMURA\textsubscript{Rubric})}  &  $\checkmark$  &  &  0.700 &  0.914 &  0.378 &  9.2  & $\checkmark$  &  & 0.591 &   0.853 &  0.317 &  16.3&   $\checkmark$ &  &   0.620& 0.863 &  0.260 &  13.1\\
        \textbf{Ours (HOMURA\textsubscript{Reason})}  &  $\checkmark$  &  &  0.701 &  0.925 &  0.376 & 10.1& $\checkmark$  &  & 0.603 &   0.861 &  0.321  & 14.7&  $\checkmark$ &  &  0.605 &  0.858 &  0.309 &  13.2 \\
        \bottomrule
    \end{tabular}%
    }
    \vspace{2mm}
    
    \raggedright
    \footnotesize
    Note: IB: In Bounds, $\checkmark$ indicates within bounds, $\times$ indicates out of bounds. AVG-Tokens: Average number of output tokens per sample; for reasoning models ($^*$), values in parentheses denote the total tokens consumed (including internal thinking).

    \vspace{-4mm}
\end{table*}
